Efficient NTK using Dimensionality Reduction

Recently, neural tangent kernel (NTK) has been used to explain the dynamics of learning parameters of neural networks, at the large width limit. Quantitative analyses of NTK give rise to network widths that are often impractical and incur high costs in time and energy in both training and deployment. Using a matrix factorization technique, we show how to obtain similar guarantees to those obtained by a prior analysis while reducing training and inference resource costs. The importance of our result further increases when the input points' data dimension is in the same order as the number of input points. More generally, our work suggests how to analyze large width networks in which dense linear layers are replaced with a low complexity factorization, thus reducing the heavy dependence on the large width.

==> reference.tex <==
@article{du2018gradient,
  title={Gradient descent provably optimizes over-parameterized neural networks},
  author={Du, Simon S and Zhai, Xiyu and Poczos, Barnabas and Singh, Aarti},
  journal={arXiv preprint arXiv:1810.02054},
  year={2018}
}

@inproceedings{arora2019fine,
  title={Fine-grained analysis of optimization and generalization for overparameterized two-layer neural networks},
  author={Arora, Sanjeev and Du, Simon and Hu, Wei and Li, Zhiyuan and Wang, Ruosong},
  booktitle={International Conference on Machine Learning},
  pages={322--332},
  year={2019},
  organization={PMLR}
}

@article{song2019quadratic,
  title={Quadratic suffices for over-parametrization via matrix chernoff bound},
  author={Song, Zhao and Yang, Xin},
  journal={arXiv preprint arXiv:1906.03593},
  year={2019}
}

@article{han2021random,
  title={Random Features for the Neural Tangent Kernel},
  author={Han, Insu and Avron, Haim and Shoham, Neta and Kim, Chaewon and Shin, Jinwoo},
  journal={arXiv preprint arXiv:2104.01351},
  year={2021}
}

@article{alemohammad2020recurrent,
  title={The recurrent neural tangent kernel},
  author={Alemohammad, Sina and Wang, Zichao and Balestriero, Randall and Baraniuk, Richard},
  journal={arXiv preprint arXiv:2006.10246},
  year={2020}
}

@inproceedings{ailon2006approximate,
  title={Approximate nearest neighbors and the fast Johnson-Lindenstrauss transform},
  author={Ailon, Nir and Chazelle, Bernard},
  booktitle={Proceedings of the thirty-eighth annual ACM symposium on Theory of computing},
  pages={557--563},
  year={2006}
}

@article{jacot2018neural,
  title={Neural tangent kernel: Convergence and generalization in neural networks},
  author={Jacot, Arthur and Gabriel, Franck and Hongler, Cl{\'e}ment},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={25},
  year={2012}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}

@article{hinton2012deep,
  title={Deep neural networks for acoustic modeling in speech recognition: The shared views of four research groups},
  author={Hinton, Geoffrey and Deng, Li and Yu, Dong and Dahl, George E and Mohamed, Abdel-rahman and Jaitly, Navdeep and Senior, Andrew and Vanhoucke, Vincent and Nguyen, Patrick and Sainath, Tara N and others},
  journal={IEEE Signal processing magazine},
  volume={29},
  number={6},
  pages={82--97},
  year={2012},
  publisher={IEEE}
}

@inproceedings{devlin2019bert,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  booktitle={Proceedings of the 2019 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
  pages={4171--4186},
  year={2019}
}

@article{collobert2011natural,
  title={Natural language processing (almost) from scratch},
  author={Collobert, Ronan and Weston, Jason and Bottou, L{\'e}on and Karlen, Michael and Kavukcuoglu, Koray and Kuksa, Pavel},
  journal={Journal of machine learning research},
  volume={12},
  number={ARTICLE},
  pages={2493--2537},
  year={2011}
}

@inproceedings{ailon2021sparse,
  title={Sparse linear networks with a fixed butterfly structure: theory and practice},
  author={Ailon, Nir and Leibovitch, Omer and Nair, Vineet},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={1174--1184},
  year={2021},
  organization={PMLR}
}

 @inproceedings{dao2019learning,
  title={Learning fast algorithms for linear transforms using butterfly factorizations},
  author={Dao, Tri and Gu, Albert and Eichhorn, Matthew and Rudra, Atri and R{\'e}, Christopher},
  booktitle={International conference on machine learning},
  pages={1517--1527},
  year={2019},
  organization={PMLR}
}

@inproceedings{strubell2019energy,
  title={Energy and Policy Considerations for Deep Learning in NLP},
  author={Strubell, Emma and Ganesh, Ananya and McCallum, Andrew},
  booktitle={Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
  pages={3645--3650},
  year={2019}
}

@inproceedings{khodak2020initialization,
  title={Initialization and Regularization of Factorized Neural Layers},
  author={Khodak, Mikhail and Tenenholtz, Neil A and Mackey, Lester and Fusi, Nicolo},
  booktitle={International Conference on Learning Representations},
  year={2020}
}

@article{johnson1984extensions,
  title={Extensions of Lipschitz mappings into a Hilbert space 26},
  author={Johnson, William B and Lindenstrauss, Joram},
  journal={Contemporary mathematics},
  volume={26},
  pages={28},
  year={1984}
}

@inproceedings{du2019gradient,
  title={Gradient descent finds global minima of deep neural networks},
  author={Du, Simon and Lee, Jason and Li, Haochuan and Wang, Liwei and Zhai, Xiyu},
  booktitle={International conference on machine learning},
  pages={1675--1685},
  year={2019},
  organization={PMLR}
}

@article{arora2019exact,
  title={On exact computation with an infinitely wide neural net},
  author={Arora, Sanjeev and Du, Simon S and Hu, Wei and Li, Zhiyuan and Salakhutdinov, Russ R and Wang, Ruosong},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  year={2019}
}

@article{mahoney2009cur,
  title={CUR matrix decompositions for improved data analysis},
  author={Mahoney, Michael W and Drineas, Petros},
  journal={Proceedings of the National Academy of Sciences},
  volume={106},
  number={3},
  pages={697--702},
  year={2009},
  publisher={National Acad Sciences}
}

@inproceedings{liberty2013simple,
  title={Simple and deterministic matrix sketching},
  author={Liberty, Edo},
  booktitle={Proceedings of the 19th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={581--588},
  year={2013}
}

@article{matouvsek2008variants,
  title={On variants of the Johnson--Lindenstrauss lemma},
  author={Matou{\v{s}}ek, Ji{\v{r}}{\'\i}},
  journal={Random Structures \& Algorithms},
  volume={33},
  number={2},
  pages={142--156},
  year={2008},
  publisher={Wiley Online Library}
}

@inproceedings{larsen2017optimality,
  title={Optimality of the Johnson-Lindenstrauss lemma},
  author={Larsen, Kasper Green and Nelson, Jelani},
  booktitle={2017 IEEE 58th Annual Symposium on Foundations of Computer Science (FOCS)},
  pages={633--638},
  year={2017},
  organization={IEEE}
}

%Entries
@article{kolda2009tensor,
  title={Tensor decompositions and applications},
  author={Kolda, Tamara G and Bader, Brett W},
  journal={SIAM review},
  volume={51},
  number={3},
  pages={455--500},
  year={2009},
  publisher={SIAM}
}


@inproceedings{badoiu2003smaller,
  title={Smaller core-sets for balls},
  author={Badoiu, Mihai and Clarkson, Kenneth L},
  booktitle={SODA},
  volume={3},
  pages={801--802},
  year={2003}
}

@article{kruskal1977three,
  title={Three-way arrays: rank and uniqueness of trilinear decompositions, with application to arithmetic complexity and statistics},
  author={Kruskal, Joseph B},
  journal={Linear algebra and its applications},
  volume={18},
  number={2},
  pages={95--138},
  year={1977},
  publisher={North-Holland}
}

@article{anandkumar2014tensor,
  title={Tensor decompositions for learning latent variable models},
  author={Anandkumar, Animashree and Ge, Rong and Hsu, Daniel and Kakade, Sham M and Telgarsky, Matus},
  journal={The Journal of Machine Learning Research},
  volume={15},
  number={1},
  pages={2773--2832},
  year={2014},
  publisher={JMLR. org}
}

@article{huang2015online,
  title={Online tensor methods for learning latent variable models},
  author={Huang, Furong and Niranjan, UN and Hakeem, Mohammad Umar and Anandkumar, Animashree},
  journal={The Journal of Machine Learning Research},
  volume={16},
  number={1},
  pages={2797--2835},
  year={2015},
  publisher={JMLR. org}
}

@article{hillar2013most,
  title={Most tensor problems are NP-hard},
  author={Hillar, Christopher J and Lim, Lek-Heng},
  journal={Journal of the ACM (JACM)},
  volume={60},
  number={6},
  pages={45},
  year={2013},
  publisher={ACM}
}

@inproceedings{cohen2016online,
  title={Online Row Sampling},
  author={Cohen, Michael B and Musco, Cameron and Pachocki, Jakub},
  booktitle={Approximation, Randomization, and Combinatorial Optimization. Algorithms and Techniques (APPROX/RANDOM 2016)},
  year={2016},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik}
}

@inproceedings{wang2016online,
  title={Online and differentially-private tensor decomposition},
  author={Wang, Yining and Anandkumar, Anima},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3531--3539},
  year={2016}
}

@article{woodruff2014sketching,
  title={Sketching as a tool for numerical linear algebra},
  author={Woodruff, David P and others},
  journal={Foundations and Trends{\textregistered} in Theoretical Computer Science},
  volume={10},
  number={1--2},
  pages={1--157},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{braverman2016new,
  title={New frameworks for offline and streaming coreset constructions},
  author={Braverman, Vladimir and Feldman, Dan and Lang, Harry},
  journal={arXiv preprint arXiv:1612.00889},
  year={2016}
}

@book{dubhashi2009concentration,
  title={Concentration of measure for the analysis of randomized algorithms},
  author={Dubhashi, Devdatt P and Panconesi, Alessandro},
  year={2009},
  publisher={Cambridge University Press}
}

@article{bachem2017practical,
  title={Practical Coreset Constructions for Machine Learning},
  author={Bachem, Olivier and Lucic, Mario and Krause, Andreas},
  journal={stat},
  volume={1050},
  pages={4},
  year={2017}
}

@inproceedings{wang2015fast,
  title={Fast and guaranteed tensor decomposition via sketching},
  author={Wang, Yining and Tung, Hsiao-Yu and Smola, Alexander J and Anandkumar, Anima},
  booktitle={Advances in Neural Information Processing Systems},
  pages={991--999},
  year={2015}
}

@inproceedings{cohen2017input,
  title={Input sparsity time low-rank approximation via ridge leverage score sampling},
  author={Cohen, Michael B and Musco, Cameron and Musco, Christopher},
  booktitle={Proceedings of the Twenty-Eighth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={1758--1777},
  year={2017},
  organization={SIAM}
}

@article{bhojanapalli2015new,
  title={A New Sampling Technique for Tensors},
  author={Bhojanapalli, Srinadh and Sanghavi, Sujay},
  journal={stat},
  volume={1050},
  pages={19},
  year={2015}
}

@inproceedings{song2016sublinear,
  title={Sublinear time orthogonal tensor decomposition},
  author={Song, Zhao and Woodruff, David and Zhang, Huan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={793--801},
  year={2016}
}

@inproceedings{song2019relative,
  title={Relative error tensor low rank approximation},
  author={Song, Zhao and Woodruff, David P and Zhong, Peilin},
  booktitle={Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms},
  pages={2772--2789},
  year={2019},
  organization={Society for Industrial and Applied Mathematics}
}

@article{harshman1970foundations,
  title={Foundations of the PARAFAC procedure: Models and conditions for an" explanatory" multimodal factor analysis},
  author={Harshman, Richard A and others},
  year={1970},
  publisher={University of California at Los Angeles Los Angeles, CA}
}

@article{sherman1950adjustment,
  title={Adjustment of an inverse matrix corresponding to a change in one element of a given matrix},
  author={Sherman, Jack and Morrison, Winifred J},
  journal={The Annals of Mathematical Statistics},
  volume={21},
  number={1},
  pages={124--127},
  year={1950},
  publisher={JSTOR}
}

@inproceedings{cohen2015uniform,
  title={Uniform sampling for matrix approximation},
  author={Cohen, Michael B and Lee, Yin Tat and Musco, Cameron and Musco, Christopher and Peng, Richard and Sidford, Aaron},
  booktitle={Proceedings of the 2015 Conference on Innovations in Theoretical Computer Science},
  pages={181--190},
  year={2015},
  organization={ACM}
}

@inproceedings{anandkumar2012method,
  title={A method of moments for mixture models and hidden Markov models},
  author={Anandkumar, Animashree and Hsu, Daniel and Kakade, Sham M},
  booktitle={Conference on Learning Theory},
  pages={33--1},
  year={2012}
}

@article{beckmann2005tensorial,
  title={Tensorial extensions of independent component analysis for multisubject FMRI analysis},
  author={Beckmann, Christian F and Smith, Stephen M},
  journal={Neuroimage},
  volume={25},
  number={1},
  pages={294--311},
  year={2005},
  publisher={Elsevier}
}

@article{dunlavy2011temporal,
  title={Temporal link prediction using matrix and tensor factorizations},
  author={Dunlavy, Daniel M and Kolda, Tamara G and Acar, Evrim},
  journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
  volume={5},
  number={2},
  pages={10},
  year={2011},
  publisher={ACM}
}

@article{hsu2012spectral,
  title={A spectral algorithm for learning hidden Markov models},
  author={Hsu, Daniel and Kakade, Sham M and Zhang, Tong},
  journal={Journal of Computer and System Sciences},
  volume={78},
  number={5},
  pages={1460--1480},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{jenatton2012latent,
  title={A latent factor model for highly multi-relational data},
  author={Jenatton, Rodolphe and Roux, Nicolas L and Bordes, Antoine and Obozinski, Guillaume R},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3167--3175},
  year={2012}
}

@inproceedings{nickel2011three,
  title={A Three-Way Model for Collective Learning on Multi-Relational Data.},
  author={Nickel, Maximilian and Tresp, Volker and Kriegel, Hans-Peter},
  booktitle={ICML},
  volume={11},
  pages={809--816},
  year={2011}
}

@inproceedings{papalexakis2013more,
  title={Do more views of a graph help? community detection and clustering in multi-graphs},
  author={Papalexakis, Evangelos E and Akoglu, Leman and Ience, Dino},
  booktitle={Proceedings of the 16th International Conference on Information FUSION},
  pages={899--905},
  year={2013},
  organization={IEEE}
}

@inproceedings{xiong2010temporal,
  title={Temporal collaborative filtering with bayesian probabilistic tensor factorization},
  author={Xiong, Liang and Chen, Xi and Huang, Tzu-Kuo and Schneider, Jeff and Carbonell, Jaime G},
  booktitle={Proceedings of the 2010 SIAM International Conference on Data Mining},
  pages={211--222},
  year={2010},
  organization={SIAM}
}

@article{sidiropoulos2017tensor,
  title={Tensor decomposition for signal processing and machine learning},
  author={Sidiropoulos, Nicholas D and De Lathauwer, Lieven and Fu, Xiao and Huang, Kejun and Papalexakis, Evangelos E and Faloutsos, Christos},
  journal={IEEE Transactions on Signal Processing},
  volume={65},
  number={13},
  pages={3551--3582},
  year={2017},
  publisher={IEEE}
}

@article{cong2015tensor,
  title={Tensor decomposition of EEG signals: a brief review},
  author={Cong, Fengyu and Lin, Qiu-Hua and Kuang, Li-Dan and Gong, Xiao-Feng and Astikainen, Piia and Ristaniemi, Tapani},
  journal={Journal of neuroscience methods},
  volume={248},
  pages={59--69},
  year={2015},
  publisher={Elsevier}
}

@article{oseledets2011tensor,
  title={Tensor-train decomposition},
  author={Oseledets, Ivan V},
  journal={SIAM Journal on Scientific Computing},
  volume={33},
  number={5},
  pages={2295--2317},
  year={2011},
  publisher={SIAM}
}

@inproceedings{feldman2011unified,
  title={A unified framework for approximating and clustering data},
  author={Feldman, Dan and Langberg, Michael},
  booktitle={Proceedings of the forty-third annual ACM symposium on Theory of computing},
  pages={569--578},
  year={2011},
  organization={ACM}
}

@inproceedings{langberg2010universal,
  title={Universal $\varepsilon$-approximators for integrals},
  author={Langberg, Michael and Schulman, Leonard J},
  booktitle={Proceedings of the twenty-first annual ACM-SIAM symposium on Discrete Algorithms},
  pages={598--607},
  year={2010},
  organization={SIAM}
}

@article{agarwal2005geometric,
  title={Geometric approximation via coresets},
  author={Agarwal, Pankaj K and Har-Peled, Sariel and Varadarajan, Kasturi R and others},
  journal={Combinatorial and computational geometry},
  volume={52},
  pages={1--30},
  year={2005},
  publisher={Cambridge University Press Cambridge, UK}
}

@inproceedings{har2004coresets,
  title={On coresets for k-means and k-median clustering},
  author={Har-Peled, Sariel and Mazumdar, Soham},
  booktitle={Proceedings of the thirty-sixth annual ACM symposium on Theory of computing},
  pages={291--300},
  year={2004},
  organization={ACM}
}

@article{vrabel2016note,
  title={A note on the Matrix Determinant Lemma},
  author={Vrabel, Robert and Bottu, J},
  journal={International Journal of Pure and Applied Mathematics},
  volume={111},
  number={4},
  pages={643--646},
  year={2016}
}

@article{janzamin2015beating,
  title={Beating the perils of non-convexity: Guaranteed training of neural networks using tensor methods},
  author={Janzamin, Majid and Sedghi, Hanie and Anandkumar, Anima},
  journal={arXiv preprint arXiv:1506.08473},
  year={2015}
}

@article{dasgupta2009sampling,
  title={Sampling algorithms and coresets for $\backslash$ell\_p regression},
  author={Dasgupta, Anirban and Drineas, Petros and Harb, Boulos and Kumar, Ravi and Mahoney, Michael W},
  journal={SIAM Journal on Computing},
  volume={38},
  number={5},
  pages={2060--2078},
  year={2009},
  publisher={SIAM}
}

@article{kremer1999randomized,
  title={On randomized one-round communication complexity},
  author={Kremer, Ilan and Nisan, Noam and Ron, Dana},
  journal={Computational Complexity},
  volume={8},
  number={1},
  pages={21--49},
  year={1999},
  publisher={Springer}
}

@article{tropp2011freedman,
  title={Freedman's inequality for matrix martingales},
  author={Tropp, Joel and others},
  journal={Electronic Communications in Probability},
  volume={16},
  pages={262--270},
  year={2011},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}

@inproceedings{dickens2018leveraging,
  title={Leveraging Well-Conditioned Bases: Streaming and Distributed Summaries in Minkowski $ p $-Norms},
  author={Dickens, Charlie and Cormode, Graham and Woodruff, David},
  booktitle={International Conference on Machine Learning},
  pages={1243--1251},
  year={2018}
}

@inproceedings{woodruff2013subspace,
  title={Subspace embeddings and $\backslash$ell\_p-regression using exponential random variables},
  author={Woodruff, David and Zhang, Qin},
  booktitle={Conference on Learning Theory},
  pages={546--567},
  year={2013}
}

@inproceedings{cohen2015p,
  title={L p row sampling by lewis weights},
  author={Cohen, Michael B and Peng, Richard},
  booktitle={Proceedings of the forty-seventh annual ACM symposium on Theory of computing},
  pages={183--192},
  year={2015},
  organization={ACM}
}

@article{tropp2015introduction,
  title={An introduction to matrix concentration inequalities},
  author={Tropp, Joel A and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={8},
  number={1-2},
  pages={1--230},
  year={2015},
  publisher={Now Publishers, Inc.}
}

@inproceedings{papailiopoulos2014provable,
  title={Provable deterministic leverage score sampling},
  author={Papailiopoulos, Dimitris and Kyrillidis, Anastasios and Boutsidis, Christos},
  booktitle={Proceedings of the 20th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={997--1006},
  year={2014},
  organization={ACM}
}

@article{clarkson2016fast,
  title={The fast cauchy transform and faster robust linear regression},
  author={Clarkson, Kenneth L and Drineas, Petros and Magdon-Ismail, Malik and Mahoney, Michael W and Meng, Xiangrui and Woodruff, David P},
  journal={SIAM Journal on Computing},
  volume={45},
  number={3},
  pages={763--810},
  year={2016},
  publisher={SIAM}
}

@inproceedings{ma2016polynomial,
  title={Polynomial-time tensor decompositions with sum-of-squares},
  author={Ma, Tengyu and Shi, Jonathan and Steurer, David},
  booktitle={2016 IEEE 57th Annual Symposium on Foundations of Computer Science (FOCS)},
  pages={438--446},
  year={2016},
  organization={IEEE}
}

@article{vervliet2016tensorlab,
  title={Tensorlab 3.0. Available online},
  author={Vervliet, N and Debals, O and Sorber, L and Van Barel, M and De Lathauwer, L},
  journal={URL: http://www. tensorlab. net},
  year={2016}
}

@article{batson2012twice,
  title={Twice-{R}amanujan {S}parsifiers},
  author={Batson, Joshua and Spielman, Daniel A and Srivastava, Nikhil},
  journal={SIAM Journal on Computing},
  volume={41},
  number={6},
  pages={1704--1721},
  year={2012},
  publisher={SIAM}
}

@article{lee2018constructing,
  title={Constructing linear-sized spectral sparsification in almost-linear time},
  author={Lee, Yin Tat and Sun, He},
  journal={SIAM Journal on Computing},
  volume={47},
  number={6},
  pages={2315--2336},
  year={2018},
  publisher={SIAM}
}

@article{ghashami2016frequent,
  title={Frequent directions: Simple and deterministic matrix sketching},
  author={Ghashami, Mina and Liberty, Edo and Phillips, Jeff M and Woodruff, David P},
  journal={SIAM Journal on Computing},
  volume={45},
  number={5},
  pages={1762--1792},
  year={2016},
  publisher={SIAM}
}

@article{janzamin2014score,
  title={Score function features for discriminative learning: Matrix and tensor framework},
  author={Janzamin, Majid and Sedghi, Hanie and Anandkumar, Anima},
  journal={arXiv preprint arXiv:1412.2863},
  year={2014}
}

@article{kachamoptimal,
  title={Optimal Deterministic Coresets for Ridge Regression},
  author={Kacham, Praneeth and Woodruff, David P}
}

@inproceedings{sedghi2016provable,
  title={Provable tensor methods for learning mixtures of generalized linear models},
  author={Sedghi, Hanie and Janzamin, Majid and Anandkumar, Anima},
  booktitle={Artificial Intelligence and Statistics},
  pages={1223--1231},
  year={2016}
}

@inproceedings{chierichetti2017algorithms,
  title={Algorithms for L\_p low-rank approximation},
  author={Chierichetti, Flavio and Gollapudi, Sreenivas and Kumar, Ravi and Lattanzi, Silvio and Panigrahy, Rina and Woodruff, David P},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={806--814},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{dan2019optimal,
  title={Optimal Analysis of Subset-Selection Based L\_p Low-Rank Approximation},
  author={Dan, Chen and Wang, Hong and Zhang, Hongyang and Zhou, Yuchen and Ravikumar, Pradeep K},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2537--2548},
  year={2019}
}

@article{schechtman2011tight,
  title={Tight embedding of subspaces of $L_{p}$ in $\ell_{p}^{n}$ for even $p$},
  author={Schechtman, Gideon},
  journal={Proceedings of the American Mathematical Society},
  volume={139},
  number={12},
  pages={4419--4421},
  year={2011}
}

@inproceedings{balcan2013distributed,
  title={Distributed $ k $-means and $ k $-median Clustering on General Topologies},
  author={Balcan, Maria-Florina F and Ehrlich, Steven and Liang, Yingyu},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1995--2003},
  year={2013}
}

@inproceedings{lucic2016strong,
  title={Strong coresets for hard and soft Bregman clustering with applications to exponential family mixtures},
  author={Lucic, Mario and Bachem, Olivier and Krause, Andreas},
  booktitle={Artificial intelligence and statistics},
  pages={1--9},
  year={2016}
}

@inproceedings{bachem2018scalable,
  title={Scalable k-means clustering via lightweight coresets},
  author={Bachem, Olivier and Lucic, Mario and Krause, Andreas},
  booktitle={Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1119--1127},
  year={2018}
}

@inproceedings{bachem2018one,
  title={One-shot coresets: The case of k-clustering},
  author={Bachem, Olivier and Lucic, Mario and Lattanzi, Silvio},
  booktitle={International conference on artificial intelligence and statistics},
  pages={784--792},
  year={2018}
}

@inproceedings{feldman2016dimensionality,
  title={Dimensionality reduction of massive sparse datasets using coresets},
  author={Feldman, Dan and Volkov, Mikhail and Rus, Daniela},
  booktitle={Advances in Neural Information Processing Systems},
  pages={2766--2774},
  year={2016}
}

@inproceedings{ackermann2009coresets,
  title={Coresets and approximate clustering for Bregman divergences},
  author={Ackermann, Marcel R and Bl{\"o}mer, Johannes},
  booktitle={Proceedings of the twentieth annual ACM-SIAM symposium on Discrete algorithms},
  pages={1088--1097},
  year={2009},
  organization={SIAM}
}

@article{feldman2020turning,
  title={Turning big data into tiny data: Constant-size coresets for k-means, PCA, and projective clustering},
  author={Feldman, Dan and Schmidt, Melanie and Sohler, Christian},
  journal={SIAM Journal on Computing},
  volume={49},
  number={3},
  pages={601--657},
  year={2020},
  publisher={SIAM}
}

@article{barger2016k,
  title={Deterministic Coresets for k-Means of Big Sparse Data},
  author={Barger, Artem and Feldman, Dan},
  journal={Algorithms},
  volume={13},
  number={4},
  pages={92},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{boutsidis2013deterministic,
  title={Deterministic feature selection for k-means clustering},
  author={Boutsidis, Christos and Magdon-Ismail, Malik},
  journal={IEEE Transactions on Information Theory},
  volume={59},
  number={9},
  pages={6099--6110},
  year={2013},
  publisher={IEEE}
}

@inproceedings{cohen2015dimensionality,
  title={Dimensionality reduction for k-means clustering and low rank approximation},
  author={Cohen, Michael B and Elder, Sam and Musco, Cameron and Musco, Christopher and Persu, Madalina},
  booktitle={Proceedings of the forty-seventh annual ACM symposium on Theory of computing},
  pages={163--172},
  year={2015}
}

@article{banerjee2005clustering,
  title={Clustering with Bregman divergences},
  author={Banerjee, Arindam and Merugu, Srujana and Dhillon, Inderjit S and Ghosh, Joydeep},
  journal={Journal of machine learning research},
  volume={6},
  number={Oct},
  pages={1705--1749},
  year={2005}
}

@inproceedings{acharyya2013bregman,
  title={Bregman divergences and triangle inequality},
  author={Acharyya, Sreangsu and Banerjee, Arindam and Boley, Daniel},
  booktitle={Proceedings of the 2013 SIAM International Conference on Data Mining},
  pages={476--484},
  year={2013},
  organization={SIAM}
}

@inproceedings{ackermann2010bregman,
  title={Bregman clustering for separable instances},
  author={Ackermann, Marcel R and Bl{\"o}mer, Johannes},
  booktitle={Scandinavian Workshop on Algorithm Theory},
  pages={212--223},
  year={2010},
  organization={Springer}
}

@inproceedings{liberty2016algorithm,
  title={An algorithm for online k-means clustering},
  author={Liberty, Edo and Sriharsha, Ram and Sviridenko, Maxim},
  booktitle={2016 Proceedings of the eighteenth workshop on algorithm engineering and experiments (ALENEX)},
  pages={81--89},
  year={2016},
  organization={SIAM}
}

@inproceedings{bhaskara2020robust,
  title={Robust Algorithms for Online $ k $-means Clustering},
  author={Bhaskara, Aditya and Rwanpathirana, Aravinda Kanchana},
  booktitle={Algorithmic Learning Theory},
  pages={148--173},
  year={2020}
}

@inproceedings{lattanzi2017consistent,
  title={Consistent k-clustering},
  author={Lattanzi, Silvio and Vassilvitskii, Sergei},
  booktitle={International Conference on Machine Learning},
  pages={1975--1984},
  year={2017}
}

@inproceedings{arthur2007k,
  title={k-means++ the advantages of careful seeding},
  author={Arthur, David and Vassilvitskii, Sergei},
  booktitle={Proceedings of the eighteenth annual ACM-SIAM symposium on Discrete algorithms},
  pages={1027--1035},
  year={2007}
}

@inproceedings{bachem2015coresets,
  title={Coresets for Nonparametric Estimation-the Case of DP-Means.},
  author={Bachem, Olivier and Lucic, Mario and Krause, Andreas},
  booktitle={ICML},
  pages={209--217},
  year={2015}
}

@inproceedings{chhaya2020coresets,
  title={On coresets for regularized regression},
  author={Chhaya, Rachit and Dasgupta, Anirban and Shit, Supratim},
  booktitle={International Conference on Machine Learning},
  pages={1866--1876},
  year={2020},
  organization={PMLR}
}

@inproceedings{huang2020coresets,
  title={Coresets for clustering in euclidean spaces: importance sampling is nearly optimal},
  author={Huang, Lingxiao and Vishnoi, Nisheeth K},
  booktitle={Proceedings of the 52nd Annual ACM SIGACT Symposium on Theory of Computing},
  pages={1416--1429},
  year={2020}
}

@inproceedings{kobren2017hierarchical,
  title={A hierarchical algorithm for extreme clustering},
  author={Kobren, Ari and Monath, Nicholas and Krishnamurthy, Akshay and McCallum, Andrew},
  booktitle={Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={255--264},
  year={2017}
}

@inproceedings{baykal2018data,
  title={Data-Dependent Coresets for Compressing Neural Networks with Applications to Generalization Bounds},
  author={Baykal, Cenk and Liebenwein, Lucas and Gilitschenski, Igor and Feldman, Dan and Rus, Daniela},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{chhaya2020streaming,
  title={Streaming coresets for symmetric tensor factorization},
  author={Chhaya, Rachit and Choudhari, Jayesh and Dasgupta, Anirban and Shit, Supratim},
  booktitle={International Conference on Machine Learning},
  pages={1855--1865},
  year={2020},
  organization={PMLR}
}

@inproceedings{bachem2017uniform,
  title={Uniform deviation bounds for k-means clustering},
  author={Bachem, Olivier and Lucic, Mario and Hassani, S Hamed and Krause, Andreas},
  booktitle={International Conference on Machine Learning},
  pages={283--291},
  year={2017},
  organization={PMLR}
}

@inproceedings{kulis2012revisiting,
  title={Revisiting k-means: new algorithms via Bayesian nonparametrics},
  author={Kulis, Brian and Jordan, Michael I},
  booktitle={Proceedings of the 29th International Coference on International Conference on Machine Learning},
  pages={1131--1138},
  year={2012}
}

@article{haussler2018decision,
  title={Decision theoretic generalizations of the PAC model for neural net and other learning applications},
  author={Haussler, David},
  journal={Information and computation},
  volume={100},
  number={1},
  pages={78--150},
  year={1992},
  publisher={Elsevier}
}

@article{biau2008performance,
  title={On the performance of clustering in Hilbert spaces},
  author={Biau, G{\'e}rard and Devroye, Luc and Lugosi, G{\'a}bor},
  journal={IEEE Transactions on Information Theory},
  volume={54},
  number={2},
  pages={781--790},
  year={2008},
  publisher={IEEE}
}

@inproceedings{cohen2016optimal,
  title={Optimal approximate matrix product in terms of stable rank},
  author={Cohen, Michael B and Nelson, Jelani and Woodruff, David P},
  booktitle={International Colloquium on Automata, Languages, and Programming},
  year={2016},
  organization={Schloss Dagstuhl-Leibniz-Zentrum fur Informatik GmbH, Dagstuhl Publishing}
}

@article{chhaya2020online,
  title={Online Coresets for Clustering with Bregman Divergences},
  author={Chhaya, Rachit and Choudhari, Jayesh and Dasgupta, Anirban and Shit, Supratim},
  year={2020}
}

@inproceedings{chhaya2022coresets,
  title={On Coresets for Fair Regression and Individually Fair Clustering},
  author={Chhaya, Rachit and Dasgupta, Anirban and Choudhari, Jayesh and Shit, Supratim},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={9603--9625},
  year={2022},
  organization={PMLR}
}

@inproceedings{kacham2020optimal,
  title={Optimal deterministic coresets for ridge regression},
  author={Kacham, Praneeth and Woodruff, David},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={4141--4150},
  year={2020},
  organization={PMLR}
}

@article{CohenAddad2022TowardsOL,
  title={Towards optimal lower bounds for k-median and k-means coresets},
  author={Vincent Cohen-Addad and Kasper Green Larsen and David Saulpic and Chris Schwiegelshohn},
  journal={Proceedings of the 54th Annual ACM SIGACT Symposium on Theory of Computing},
  year={2022}
}

@article{har2007smaller,
  title={Smaller coresets for k-median and k-means clustering},
  author={Har-Peled, Sariel and Kushal, Akash},
  journal={Discrete \& Computational Geometry},
  volume={37},
  number={1},
  pages={3--19},
  year={2007},
  publisher={Springer}
}

@inproceedings{feldman2007ptas,
  title={A PTAS for k-means clustering based on weak coresets},
  author={Feldman, Dan and Monemizadeh, Morteza and Sohler, Christian},
  booktitle={Proceedings of the twenty-third annual symposium on Computational geometry},
  pages={11--18},
  year={2007}
}

@inproceedings{feldman2013turning,
  title={Turning big data into tiny data: Constant-size coresets for k-means, pca and projective clustering},
  author={Feldman, Dan and Schmidt, Melanie and Sohler, Christian},
  booktitle={Proceedings of the twenty-fourth annual ACM-SIAM symposium on Discrete algorithms},
  pages={1434--1453},
  year={2013},
  organization={SIAM}
}

@article{jiang2021coresets,
  title={Coresets for Clustering with Missing Values},
  author={Jiang, Shaofeng and Krauthgamer, Robert and Wu, Xuan and others},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@inproceedings{tukan2022new,
  title={New Coresets for Projective Clustering and Applications},
  author={Tukan, Murad and Wu, Xuan and Zhou, Samson and Braverman, Vladimir and Feldman, Dan},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={5391--5415},
  year={2022},
  organization={PMLR}
}

@inproceedings{munteanu2018coresets,
  title={On coresets for logistic regression},
  author={Munteanu, Alexander and Schwiegelshohn, Chris and Sohler, Christian and Woodruff, David},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6561--6570},
  year={2018}
}

@article{tukan2020coresets,
  title={Coresets for near-convex functions},
  author={Tukan, Morad and Maalouf, Alaa and Feldman, Dan},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}

@inproceedings{munteanu2021oblivious,
  title={Oblivious sketching for logistic regression},
  author={Munteanu, Alexander and Omlor, Simon and Woodruff, David},
  booktitle={International Conference on Machine Learning},
  pages={7861--7871},
  year={2021},
  organization={PMLR}
}

@inproceedings{zheng2017coresets,
  title={Coresets for kernel regression},
  author={Zheng, Yan and Phillips, Jeff M},
  booktitle={Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={645--654},
  year={2017}
}

@article{mai2021coresets,
  title={Coresets for classification--simplified and strengthened},
  author={Mai, Tung and Musco, Cameron and Rao, Anup},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={11643--11654},
  year={2021}
}

@article{drineas2012fast,
  title={Fast approximation of matrix coherence and statistical leverage},
  author={Drineas, Petros and Magdon-Ismail, Malik and Mahoney, Michael W and Woodruff, David P},
  journal={The Journal of Machine Learning Research},
  volume={13},
  number={1},
  pages={3475--3506},
  year={2012},
  publisher={JMLR. org}
}

@article{huggins2016coresets,
  title={Coresets for scalable Bayesian logistic regression},
  author={Huggins, Jonathan and Campbell, Trevor and Broderick, Tamara},
  journal={Advances in Neural Information Processing Systems},
  volume={29},
  year={2016}
}

@inproceedings{sener2017active,
  title={Active Learning for Convolutional Neural Networks: A Core-Set Approach},
  author={Sener, Ozan and Savarese, Silvio},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{tolochinsky2018coresets,
  title={Generic coreset for scalable learning of monotonic kernels: Logistic regression, sigmoid and more},
  author={Tolochinksy, Elad and Jubran, Ibrahim and Feldman, Dan},
  booktitle={International Conference on Machine Learning},
  pages={21520--21547},
  year={2022},
  organization={PMLR}
}

@inproceedings{mussay2019data,
  title={Data-Independent Neural Pruning via Coresets},
  author={Mussay, Ben and Osadchy, Margarita and Braverman, Vladimir and Zhou, Samson and Feldman, Dan},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@article{mirzasoleiman2020coresets,
  title={Coresets for Robust Training of Neural Networks against Noisy Labels},
  author={Mirzasoleiman, Baharan and Cao, Kaidi and Leskovec, Jure},
  journal={Neural Information Processing Systems (NeurIPS)},
  year={2020}
}

@inproceedings{dubey2018coreset,
  title={Coreset-based neural network compression},
  author={Dubey, Abhimanyu and Chatterjee, Moitreya and Ahuja, Narendra},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={454--470},
  year={2018}
}

@article{jubran2021overview,
  title={Overview of accurate coresets},
  author={Jubran, Ibrahim and Maalouf, Alaa and Feldman, Dan},
  journal={Wiley Interdisciplinary Reviews: Data Mining and Knowledge Discovery},
  volume={11},
  number={6},
  pages={e1429},
  year={2021},
  publisher={Wiley Online Library}
}

@inproceedings{har2005smaller,
  title={Smaller coresets for k-median and k-means clustering},
  author={Har-Peled, Sariel and Kushal, Akash},
  booktitle={Proceedings of the twenty-first annual symposium on Computational geometry},
  pages={126--134},
  year={2005}
}

@article{chen2009coresets,
  title={On coresets for k-median and k-means clustering in metric and euclidean spaces and their applications},
  author={Chen, Ke},
  journal={SIAM Journal on Computing},
  volume={39},
  number={3},
  pages={923--947},
  year={2009},
  publisher={SIAM}
}

@inproceedings{sohler2018strong,
  title={Strong coresets for k-median and subspace approximation: Goodbye dimension},
  author={Sohler, Christian and Woodruff, David P},
  booktitle={2018 IEEE 59th Annual Symposium on Foundations of Computer Science (FOCS)},
  pages={802--813},
  year={2018},
  organization={IEEE}
}

@inproceedings{becchetti2019oblivious,
  title={Oblivious dimension reduction for k-means: beyond subspaces and the Johnson-Lindenstrauss lemma},
  author={Becchetti, Luca and Bury, Marc and Cohen-Addad, Vincent and Grandoni, Fabrizio and Schwiegelshohn, Chris},
  booktitle={Proceedings of the 51st annual ACM SIGACT symposium on theory of computing},
  pages={1039--1050},
  year={2019}
}

@inproceedings{braverman2021coresets,
  title={Coresets for clustering in excluded-minor graphs and beyond},
  author={Braverman, Vladimir and Jiang, Shaofeng H-C and Krauthgamer, Robert and Wu, Xuan},
  booktitle={Proceedings of the 2021 ACM-SIAM Symposium on Discrete Algorithms (SODA)},
  pages={2679--2696},
  year={2021},
  organization={SIAM}
}

@inproceedings{cohen2021new,
  title={A new coreset framework for clustering},
  author={Cohen-Addad, Vincent and Saulpic, David and Schwiegelshohn, Chris},
  booktitle={Proceedings of the 53rd Annual ACM SIGACT Symposium on Theory of Computing},
  pages={169--182},
  year={2021}
}

@article{shitonline,
  title={Online Coresets for Parameteric and Non-Parametric Bregman Clustering},
  author={Shit, Supratim and Dasgupta, Anirban and Chhaya, Rachit and Choudhari, Jayesh},
  journal={TMLR},
  year={2022}
}

@article{drineas2011faster,
  title={Faster least squares approximation},
  author={Drineas, Petros and Mahoney, Michael W and Muthukrishnan, Shan and Sarl{\'o}s, Tam{\'a}s},
  journal={Numerische mathematik},
  volume={117},
  number={2},
  pages={219--249},
  year={2011},
  publisher={Springer}
}

@article{ailon2010faster,
  title={Faster dimension reduction},
  author={Ailon, Nir and Chazelle, Bernard},
  journal={Communications of the ACM},
  volume={53},
  number={2},
  pages={97--104},
  year={2010},
  publisher={ACM New York, NY, USA}
}

@incollection{shit2021Lp,
  title={Lp Subspace Embedding in Input Sparsity Time},
  author={Shit, Supratim},
  booktitle={8th ACM IKDD CODS and 26th COMAD},
  pages={418--418},
  year={2021}
}

==> sections/generalize.tex <==
\subsection{Generalization}
Now for the same network we analyze how well the model generalizes for a distribution of inputs. Let $\*F(t) \in \~R^{k\ell \times n}$ defined as follows,
\begin{equation*}
\*F(t) = \frac{1}{\sqrt{m}}
\begin{pmatrix}
\mbox{vec}(\*A^{T}\*Z_{1}^{T}(t)\*X_{1}\*C^{T}) & \ldots & \mbox{vec}(\*A^{T}\*Z_{n}^{T}(t)\*X_{n}\*C^{T})
\end{pmatrix}.
\end{equation*}
For a matrix $\*B \in \~R^{k \times \ell}$, $\mbox{vec}(\*B) \in \~R^{k\ell}$ is a vector representation of the matrix $\*B$. At each iteration $t$ we get the following, 
\begin{equation*}
  \mbox{vec}(\*B(t+1)) = \mbox{vec}(\*B(t)) - \eta\*F(t)(\*u(t) - \*y).
\end{equation*}

In the following lemma we show that the matrices $\*H$ and $\*Z$ do not change much for a sufficiently large $m$.
\begin{lemma}
 Under random initialization of $\*B(0)$, for all $t > 0$ with atleast $1-2\delta$ probability we have,
 \begin{eqnarray*}
  \|\*H(t) - \*H(0)\| &=& O\left(\frac{n^{3}}{\sqrt{m}\delta^{7/2}\lambda_{0}}\right) \\
  \|\*F(t) - \*F(0)\| &=& O\left(\sqrt{\frac{n^{2}}{\sqrt{m}\delta^{5/2}\lambda_{0}}}\right) \\
 \end{eqnarray*}
\end{lemma}

\begin{proof}
 Let $R = \frac{n}{\sqrt{m}\lambda_{0}\delta^{3/2}}$. By Theorem \ref{thm:train} know that with at, $\|\*A_{r}\*B(t)\*C - \*A_{r}\*B(0)\*C\| \leq R, \forall r \in [m]$. So, by the lemma \ref{lemma:ConditionalEvent} we have, $\|\*H(t) - \*H(0)\| \leq O\left(\frac{n^{3}}{\sqrt{m}\delta^{7/2}\lambda_{0}}\right)$ with at least $1-\delta$ probability.
 
 Now we bound $\|\*F(t) - \*F(0)\|$. We first bound $\|\*A^{T}\*Z_{i}^{T}(t)\*X_{i}\*C^{T} - \*A^{T}\*Z_{i}^{T}(0)\*X_{i}\*C^{T}\|^{2}$. 
 \begin{eqnarray*}
  \|\*A^{T}\*Z_{i}^{T}(t)\*X_{i}\*C^{T} - \*A^{T}\*Z_{i}^{T}(0)\*X_{i}\*C^{T}\|^{2} &=& \|(\*A^{T}\*Z_{i}^{T}(t) - \*A^{T}\*Z_{i}^{T}(0))\*X_{i}\*C^{T}\|^{2} \\
  &\leq& \|\*A^{T}\*Z_{i}^{T}(t) - \*A^{T}\*Z_{i}^{T}(0)\|^{2}\|\*X_{i}\*C^{T}\|^{2} \\
  &\leq& O\left(\frac{mR}{\delta}\right) \\
  &=& O\left(\frac{\sqrt{m}n}{\delta^{5/2}\lambda_{0}}\right).
 \end{eqnarray*}
 The last inequality is by similar arguments in lemma \ref{lemma:ConditionalEvent}. Here we have that $\|\*Z_{i}(t) - \*Z_{i}(0)\|^{2} \leq \frac{mR}{\delta}$ with at least $1-\delta$ probability. Further, $\*A$ being a subspace preserving matrix (JL transformation) we get the final inequality. Now we have,
 \begin{eqnarray*}
  \|\*F(t) - \*F(0)\|^{2} &\leq& \sum_{i \leq n} \frac{1}{m}\|\*A^{T}\*Z_{i}^{T}(t)\*X_{i}\*C^{T} - \*A^{T}\*Z_{i}^{T}(0)\*X_{i}\*C^{T}\|^{2} \\
  &\leq& \sum_{i \leq n}O\left(\frac{\sqrt{m}n}{m\delta^{5/2}\lambda_{0}}\right) = O\left(\frac{n^{2}}{\sqrt{m}\delta^{5/2}\lambda_{0}}\right)
 \end{eqnarray*}
\end{proof}

% For all $i, j \in [n]$ every term, $\*H_{i,j}(0)$ is a random variables in $[0,O(1)]$. So using Hoeffding inequality we have $\|\*H^{\infty} - \*H(0)\|^{2} \leq \frac{n^{2}\log(n/\delta)}{2m}$ with at least $1-\delta$ probability. 
Now we present a theorem which bounds the training loss in terms of the eigen pairs of the neural tangent kernel and the response vector. 
\begin{theorem}{\label{thm:epairTrain}}
 Let $m = \Omega(\frac{n^{7}}{\lambda_{0}^{4}\delta^{4}}), \lambda_{0} = \lambda_{\min}(\*H^{\infty})$ and $(\lambda_{i}, \xi_{i})$ are the eigenpair of $\*H^{\infty}$ then for $t > 0$,
 \begin{equation*}
   \|\*y - \*u(t)\| = \sqrt{\sum_{i \leq n}(1-\eta\lambda_{i})^{2k}(\xi_{i}^{T}\*y)^{2}} \pm \varepsilon
 \end{equation*}
\end{theorem}

\begin{proof}{\label{proof:epairTrain}}
We know that, $\*u_{i}(t+1) - \*u_{i}(t) = \*I_{1}^{i} + \*I_{2}^{i}$, where $|\*I_{2}^{i}| \leq \eta\sqrt{\frac{n}{\delta}}\|\*y-\*u(t)\|$ and $\*I_{1}^{i} = -\eta\sum_{j \leq n}(\*u_{j}(t) - \*y_{j})(\*H_{i,j}(t) - \*H_{i,j}^{\perp})$. So we have, $\|\*H^{\perp}(\*u(t) - \*y)\| \leq \frac{\eta\sqrt{n}|\*S_{i}^{\perp}|}{m}\|\*u(t) - \*y\|$. This gives us, $\*u(t+1) - \*u(t) = -\eta\*H(t) + \xi(t)$ where,
\begin{eqnarray*}
 \|\xi(t)\| &=& 2\eta\frac{\sqrt{n}|\*S_{i}^{\perp}|}{md}\|\*u(t) - \*y\| \\
 &=& O\left(\eta\frac{\sqrt{n}mR}{md}\|\*u(t) - \*y\|\right) \\
 &=& O\left(\frac{\eta n^{5/2}}{\sqrt{m}d^{2}\lambda_{0}\delta}\|\*u(t) - \*y\|\right)
\end{eqnarray*}

Further, 
\begin{equation}{\label{eq:output}}
  \*u(t+1) - \*u(t) = -\eta\*H^{\infty}(\*u(t) - \*y) + \zeta(t)
\end{equation}
where $\zeta(t) = \eta(\*H^{\infty} - \*H(t))(\*u(t) - \*y) + \xi(t)$. 

Note that $\|\*H^{\infty} - \*H(t)\| \leq \|\*H^{\infty} - \*H(0)\| + \|\*H(0) - \*H(t)\| = O\left(\frac{n^{3}}{\sqrt{m}d^{2}\lambda_{0}\delta}\right)$. So, $\|\zeta(t)\| = O\left(\frac{\eta n^{3}}{\sqrt{m}d^{2}\lambda_{0}\delta}\right)\|\*u(t) - \*y\|$. Now applying \eqref{eq:output} recursively we get,
\begin{eqnarray*}
 \*u(t+1) - \*y &=& (\*I - \eta\*H^{\infty})^{t}(\*u(0) - \*y) + \sum_{t'<t} (\*I - \eta\*H^{\infty})^{t'}\zeta(t-t'-1) \\
 &=& -(\*I - \eta\*H^{\infty})^{t}\*y + (\*I - \eta\*H^{\infty})^{t}\*u(0) + \sum_{t'<t} (\*I - \eta\*H^{\infty})^{t'}\zeta(t-t'-1)
\end{eqnarray*}

Now $\|\*H^{\infty}\| \leq \mbox{tr}(\*H^{\infty}) \leq \frac{n}{2d}$ and $\eta = \frac{d^{2}\lambda_{0}}{n^{2}} = \frac{\lambda_{0}}{\|\*H^{\infty}\|^{2}} \leq \frac{1}{\|\*H^{\infty}\|}$. So, $(\*I - \eta\*H^{\infty}) \succ \*0$. Therefore,
\begin{equation*}
  \|-(\*I - \eta\*H^{\infty})^{t}\*y\| = \sqrt{\sum_{i \leq n}(1-\eta\lambda_{i})^{2k}(\chi_{i}^{T}\*y)^{2}}
\end{equation*}

Now for the second term,
\begin{equation*}
  \|(\*I - \*H^{\infty})\*u(0)\| \leq \|\*I - \*H^{\infty}\|\|\*u(0)\| \leq (1-\eta\lambda_{0})^{t}O\left(\frac{\sqrt{n}}{\delta}\right)
\end{equation*}

In the last inequality we used the fact that every $u_{i}(0)$ are bounded. So by using Markov with at least $1-\delta$ probability we have $\|\*u(0)\| \leq \frac{C\sqrt{n}}{\delta}$. 

Finally for the last term, note that we have $\|\*u(t) - \*y\| \leq (1-\eta\lambda_{0})^{t}\|\*u(0) - \*y| \leq (1-\eta\lambda_{0})^{t}\frac{\sqrt{n}}{\delta}$. So,
\begin{eqnarray*}
 \|\sum_{t'<t} (\*I - \eta\*H^{\infty})^{t'} \zeta(t-t' - 1)\| &\leq& \|\sum_{t'<t} (\*I - \eta\*H^{\infty})^{t'}\|\cdot\|\zeta(t-t' - 1)\| \\
 &\leq& \|\sum_{t'<t} (1 - \eta\lambda_{0})^{t'}\|\cdot O\left(\frac{\eta n^{3}}{\sqrt{m}d^{2}\lambda_{0}\delta}\right)\|\*u(t-t' - 1) - \*y\| \\
 &\leq& \|\sum_{t'<t} (1 - \eta\lambda_{0})^{t'}\|\cdot O\left(\frac{\eta n^{3}}{\sqrt{m}d^{2}\lambda_{0}\delta}\right)(1-\eta\lambda_{0})^{(t-t'-1)}\frac{\sqrt{n}}{\delta} \\
 &\leq& k(1 - \eta\lambda_{0})^{k-1}O\left(\frac{\eta n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{2}}\right)
\end{eqnarray*}

So we have,
\begin{eqnarray}
 \|\*u(t) - \*y\| &=& \sqrt{\sum_{i \leq n}(1-\eta\lambda_{i})^{2k}(\chi_{i}^{T}\*y)^{2}} \nonumber \\
 &\pm& O\left((1-\eta\lambda_{0})^{t}\frac{\sqrt{n}}{\delta} + k(1 - \eta\lambda_{0})^{k-1}\frac{\eta n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{2}}\right) \nonumber \\
 &=& \sqrt{\sum_{i \leq n}(1-\eta\lambda_{i})^{2k}(\chi_{i}^{T}\*y)^{2}} \nonumber \\
 &\pm& O\left((1-\eta\lambda_{0})^{t}\frac{\sqrt{n}}{\delta} + \frac{1}{\eta\lambda_{0}}\frac{\eta n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{2}}\right) \nonumber \\
 &=& \sqrt{\sum_{i \leq n}(1-\eta\lambda_{i})^{2k}(\chi_{i}^{T}\*y)^{2}} \nonumber \\
 &\pm& O\left((1-\eta\lambda_{0})^{t}\frac{\sqrt{n}}{\delta} + \frac{n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}^{2}\delta^{2}}\right)
\end{eqnarray}

Here we have used $\max_{t} k(1-\eta\lambda_{0})^{t} = O(\frac{1}{\eta\lambda_{0}})$.
 
\end{proof}

Next we show that, during the gradient descent $\*B(t)$ does not change much. As a result $\*W(t)$ does not differ much from $\*W(0)$. Let $\mbox{vec}(\*B(t+1)) \in \~R^{m\ell}$ is the vector representation of the matrix $\*B(t+1)$. Due to gradient descent we have,
\begin{equation*}
  \mbox{vec}(\*B(t+1)) = \mbox{vec}(\*B(t+1)) - \eta\*Z(t)(\*u(t) - \*y).
\end{equation*}

\begin{lemma}
 Let $m \geq \mbox{poly}(n,d^{-1},\lambda^{-1},\delta^{-1})$ and $\eta = O\left(\frac{d^{2}\lambda_{0}}{n^{2}}\right)$ then with probability at least $1-\delta$, $\|\*B(t) - \*B(0)\| \leq \sqrt{(\*y - \*u(0))^{T}(\*H^{\infty})^{-1}(\*y - \*u(0))} + \frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}}$.
\end{lemma}

\begin{proof}
 We know that $\mbox{vec}(\*B(t+1)) = \mbox{vec}(\*B(t+1)) - \eta\*Z(t)(\*u(t) - \*y)$ and $\*u(t) - \*y = -(\*I - \eta\*H^{\infty})^{t}\*y + \*e(t)$. Then,
 \begin{eqnarray*}
  \mbox{vec}(\*B(t)) - \mbox{vec}(\*B(0)) &=& \sum_{t'<t} \mbox{vec}(\*B(t'+1)) - \mbox{vec}(\*B(t')) \\
  &=& -\sum_{t'<t}\eta\*Z(t')(\*u(t') - \*y) \\
  &=& \sum_{t'<t}\eta\*Z(t')((\*I - \eta\*H^{\infty})^{t'}\*y + \*e(t)) \\
  &=& \sum_{t'<t}\eta\*Z(0)(\*I - \eta\*H^{\infty})^{t'}\*y + \sum_{t'<t}\eta(\*Z(t) - \*Z(0))(\*I - \eta\*H^{\infty})^{t'}\*y \\
  &-& \sum_{t'<t}\eta\*Z(t')\*e(t)) \\
 \end{eqnarray*}
 
 First we bound the second term. We already know that $\|\*Z(t) - \*Z(0)\| = O\left(\sqrt{\frac{n^{2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{3/2}}}\right)$. So,
 \begin{eqnarray*}
  \|\sum_{t'<t}\eta(\*Z(t) - \*Z(0))(\*I - \eta\*H^{\infty})^{t'}\*y\| &\leq& \sum_{t'<t}\eta\|\*Z(t) - \*Z(0)\| \cdot \|(\*I - \eta\*H^{\infty})^{t'}\| \cdot \|\*y\| \\
  &\leq& \frac{\eta n}{d\sqrt{\sqrt{m}\lambda_{0}\delta^{3/2}}} \sum_{t'<t} (1-\eta\lambda_{0})^{t'} \sqrt{n} \\
  &\leq& \frac{\eta n}{d\sqrt{\sqrt{m}\lambda_{0}\delta^{3/2}}} \sum_{k' = 0}^{\infty} (1-\eta\lambda_{0})^{t'} \sqrt{n} \\
  &\leq& \frac{\eta n}{d\sqrt{\sqrt{m}\lambda_{0}\delta^{3/2}}} \frac{1}{\eta\lambda_{0})} \sqrt{n} \\
  &\leq& \frac{n^{3/2}}{d\sqrt{\sqrt{m}\lambda_{0}^{3}\delta^{3/2}}}
 \end{eqnarray*}
 
 Next we bound the third term. Note that $\|\*Z(t)\| \leq \sqrt{\frac{n}{d}}$,
 \begin{eqnarray*}
  \|\sum_{t'<t}\eta\*Z(t')\*e(t))\| &\leq& \sum_{t'<t} \eta \sqrt{\frac{n}{d}}\left((1-\eta\lambda_{0})^{t'}\frac{\sqrt{n}}{\delta} + k'(1 - \eta\lambda_{0})^{k'-1}\frac{\eta n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{2}}\right) \\
  &\leq& \sum_{t'<t} \eta \sqrt{\frac{n}{d}}(1-\eta\lambda_{0})^{t'}\frac{\sqrt{n}}{\delta} + \sum_{t'<t}\eta \sqrt{\frac{n}{d}}k'(1 - \eta\lambda_{0})^{k'-1}\frac{\eta n^{7/2}}{\sqrt{m}d^{2}\lambda_{0}\delta^{2}} \\
  &\leq& \frac{n}{\sqrt{d}\lambda_{0}\delta} + \frac{\eta n^{4}}{\sqrt{m}d^{5/2}\lambda_{0}\delta^{2}}
 \end{eqnarray*}
 
 
 Noe let $\*T = \eta\sum_{t'<t}(\*I - \eta\*H^{\infty})^{t'}$ then the first term,
 \begin{eqnarray*}
  \|\sum_{t'<t}\eta\*Z(0)(\*I - \eta\*H^{\infty})^{t'}\*y\|^{2} &=& \|\*Z(0)\*T\*y\|^{2} \\
  &=& \*y^{T}\*T\*Z(0)^{T}\*Z(0)\*T\*y \\
  &=& \*y^{T}\*T\*H(0)\*T\*y \\
  &=& \*y^{T}\*T(\*H^{\infty} + \*H(0) - \*H^{\infty})\*T\*y \\
  &=& \*y^{T}\*T\*H^{\infty}\*T\*y + \*y^{T}\*T(\*H(0) - \*H^{\infty})\*T\*y \\
  &=& \*y^{T}\*T\*H^{\infty}\*T\*y + \|\*H(0) - \*H^{\infty}\|(\|\*T\|\|\*y\|)^{2} \\
  &=& \*y^{T}\*T\*H^{\infty}\*T\*y + n\sqrt{\frac{\log(n/\delta)}{md}}\left(\eta\sum_{t'<t}(1-\eta \lambda_{0})^{t'}\right)^{2} \cdot n \\
  &\leq& \*y^{T}\*T\*H^{\infty}\*T\*y + n^{2}\sqrt{\frac{\log(n/\delta)}{md\lambda_{0}^{4}}}
 \end{eqnarray*}
 
 Let $(\lambda_{i},\chi_{i})$ are the eigenpairs of $\*H^{\infty}$ then,
 \begin{equation*}
   \*T = \sum_{t'<t} \eta \sum_{i \leq n} (1-\eta\lambda_{i})^{t'}\chi_{i}\chi_{i}^{T} \leq \sum_{i \leq n} \eta \sum_{k' = 0}^{\infty}(1-\eta\lambda_{i})^{t'}\chi_{i}\chi_{i}^{T} = \sum_{i \leq n}\frac{1}{\lambda_{i}}\chi_{i}\chi_{i}^{T}.
 \end{equation*}
 
 So finally combining all we get,
 \begin{eqnarray*}
   \|\*B(t) - \*B(0)\| &\leq& \sqrt{\*y^{T}(\*H^{\infty})^{-1}\*y} + n\left(\frac{\log(n/\delta)}{md\lambda_{0}^{4}}\right)^{1/4} + \frac{n^{3/2}}{d\sqrt{\sqrt{m}\lambda_{0}^{3}\delta^{3/2}}} + \frac{n}{\sqrt{d}\lambda_{0}\delta} + \frac{\eta n^{4}}{\sqrt{m}d^{5/2}\lambda_{0}\delta^{2}} \\
   &\leq& \sqrt{\*y^{T}(\*H^{\infty})^{-1}\*y} + \frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}}
 \end{eqnarray*}
\end{proof}

\begin{lemma}
 Given $R > 0$, with probability at least $1-\delta$ over the random initialization of $\*B(0)$, simultaneously for every $\tau > 0$ the following function class,
 \begin{equation*}
  \@{F}_{R,\tau}^{\*B(0)} = \{f_{\*B,\*C,\*v}: \|\*w_{r} - \*w_{0}\| \leq R \forall r \in [m], \|\*B - \*B(0)\| \leq \tau\}
 \end{equation*}
 has empirical Rademacher complexity bounded as:
 \begin{eqnarray*}
  \@{R}_{S}(\@{F}_{R,\tau}^{\*B(0)}) &=& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}}\sum_{i \leq n} \varepsilon_{i}f(\*x_{i})\right] \\
  &\leq& \frac{\tau}{\sqrt{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)}
 \end{eqnarray*}
\end{lemma}

\begin{proof}
 We have,
 \begin{eqnarray*}
  \@{R}_{S}(\@{F}_{R,\tau}^{\*B(0)}) &=& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}}\sum_{i \leq n} \varepsilon_{i}f(\*x_{i})\right] \\
  &=& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}} \sum_{i \leq n} \varepsilon_{i}\sum_{r \leq m} \frac{v_{r}\sigma(\*w_{r}^{T}\*x_{i})}{\sqrt{m}}\right]
 \end{eqnarray*}
 
 Now, since we are only interested in $\*B$ such that $\|\*w_{r} - \*w_{r}(0)\| \leq R$, for all $r \in [m]$, if $\mathbbm{1}\{A_{r,i}\} = 0$ we must have $\mathbbm{1}\{\*w_{r}^{T}\*x_{i}\} = \mathbbm{1}\{\*w_{r}^{T}(0)\*x_{i} \geq 0\} = \mathbbm{1}_{r,i}(0)$. So, $\sigma(\*w_{r}^{T}\*x_{i}) = \mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i}$. Then we have $\sum_{i \leq n} \varepsilon_{i} \sum_{r \leq m} v_{r}\left(\sigma(\*w_{r}^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i}\right)$ as,
 \begin{eqnarray*}
  &=& \sum_{i \leq n} \varepsilon_{i} \sum_{r \leq m} (\mathbbm{1}\{A_{r,i}\} + \mathbbm{1}\{\neg A_{r,i}\})v_{r}(\sigma(\*w_{r}^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i}) \\
  &=& \sum_{i \leq n} \varepsilon_{i} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\}v_{r}(\sigma(\*w_{r}^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i}) \\
  &=& \sum_{i \leq n} \varepsilon_{i} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\}v_{r}(\sigma(\*w_{r}^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)\*w_{r}(0)^{T}\*x_{i} - \mathbbm{1}_{r,i}(0)(\*w_{r} - \*w_{r}(0))^{T}\*x_{i}) \\ 
  &=& \sum_{i \leq n} \varepsilon_{i} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\}v_{r}(\sigma(\*w_{r}^{T}\*x_{i}) - \sigma(\*w_{r}(0)^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)(\*w_{r} - \*w_{r}(0))^{T}\*x_{i}) \\
  &\leq& 2\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\}R
 \end{eqnarray*}
 
 Now we have,
 \begin{eqnarray*}
  \@{R}_{S}(\@{F}_{R,\tau}^{\*B(0)}) &=& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}} \sum_{i \leq n} \varepsilon_{i}\sum_{r \leq m} \frac{v_{r}\sigma_{\*b_{r}^{T}\*C\*x_{i}^{T}}}{\sqrt{m}}\right] \\
  &=& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}} \sum_{i \leq n} \varepsilon_{i}\sum_{r \leq m} \frac{v_{r}(\mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i} + \sigma(\*w_{r}^{T}\*x_{i}) - \mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i})}{\sqrt{m}}\right] \\
  &\leq& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{f \in \@{F}_{R,\tau}^{\*B(0)}} \sum_{i \leq n} \varepsilon_{i}\sum_{r \leq m} \frac{v_{r}\mathbbm{1}_{r,i}(0)\*w_{r}^{T}\*x_{i}}{\sqrt{m}}\right] + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \\
  &\leq& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{\*B: \|\*B - \*B(0)\| \leq \tau} \sum_{i \leq n} \varepsilon_{i}\sum_{r \leq m} \frac{v_{r}\mathbbm{1}_{r,i}(0)\*b_{r}^{T}\*C\*x_{i}^{T}}{\sqrt{m}}\right] + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \\
  &\leq& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{\*B: \|\*B - \*B(0)\| \leq \tau} \mbox{vec}(\*B)^{T}\*Z(0)\varepsilon\right] + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \\
  &\leq& \frac{1}{n}\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\sup_{\*B: \|\*B - \*B(0)\| \leq \tau} \mbox{vec}(\*B - \*B(0))^{T}\*Z(0)\varepsilon\right] + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \\
  &\leq& \frac{\tau}{n}\sqrt{\~E_{\varepsilon \in \{\pm1\}^{n}}\left[\|\*Z(0)\varepsilon\|^{2}\right]} + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \\
  &\leq& \frac{\tau}{n}\|\*Z(0)\| + \frac{2R}{n\sqrt{m}}\sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\}
 \end{eqnarray*}
 
 Next we bound $\|\*Z(0)\|$. Note that $\~E[\sum_{i \leq n}\mathbbm{1}_{r,i}(0)] = n/2$ and $\|\*Z(0)\| \leq \frac{1}{md}\sum_{r \leq m} \sum_{i \leq n} \mathbbm{1}_{r,i}(0)$. So by Hoeffding's inequality with at least $1-\delta/2$ probability,
 \begin{equation*}
   \|\*Z(0)\|^{2} \leq \frac{n}{d}\left(\frac{1}{2} + \sqrt{\frac{\log(2/\delta)}{2m}}\right)
 \end{equation*}
 
 Further, $\~E[\sum_{i \leq n} \mathbbm{1}\{A_{r,i}\}] = \frac{nR}{\sqrt{2\pi}}$. So by applying Hoeffding we have the following with at least $1-\delta/2$ probability,
 \begin{equation*}
   \sum_{i \leq n} \sum_{r \leq m} \mathbbm{1}\{A_{r,i}\} \leq mn\left(\frac{R}{\sqrt{2\pi}} + \sqrt{\frac{\log(2/\delta)}{2m}}\right)
 \end{equation*}
 
 So with probability at least $1-\delta$ we the following on the Rademacher Complexity,
 \begin{eqnarray}
  \@{R}_{S}(\@{F}_{R,\tau}^{\*B(0)}) &\leq& \frac{\tau}{n}\sqrt{\left(\frac{n}{d}\left(\frac{1}{2} + \sqrt{\frac{\log(2/\delta)}{2m}}\right)\right)} + \frac{2R}{n\sqrt{m}}mn\left(\frac{R}{\sqrt{2\pi}} + \sqrt{\frac{\log(2/\delta)}{2m}}\right) \nonumber \\
  &\leq& \frac{\tau}{n}\left(\sqrt{\frac{n}{d}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right)\right) + \frac{2R}{n\sqrt{m}}mn\left(\frac{R}{\sqrt{2\pi}} + \sqrt{\frac{\log(2/\delta)}{2m}}\right) \nonumber \\
  &\leq& \frac{\tau}{\sqrt{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)} \nonumber
 \end{eqnarray}
\end{proof}

\begin{lemma}
 Fix a failure probability $\delta \in (0,1)$, let $\@{S} = \{\*x_{i},y_{i}\}_{i = 1}^{n}$ are independent and identically distributed samples from $\@{D}$ and $m = \Omega()$. Then the neural network trained by gradient descent for $k = \Omega(\frac{1}{\eta\lambda_{0}}\log(n))$ has,
 \begin{equation*}
   \@{L}_{\@{D}} = \~E_{(\*x_{i},y_{i}) \sim \@{D}}[|u_{i}(t) - y_i|] \leq \sqrt{\frac{(\*y - \*u(0))^{T}(\*H^{\infty})^{-1}(\*y - \*u(0))}{nd}} + 
 \end{equation*}
\end{lemma}

\begin{proof}
 For the distribution $\@{D}$, let $\lambda_{\min}(\*H^{\infty}) \geq \lambda_{0}$. Now,
 \begin{eqnarray}
  \@{L}_{\@{S}}(t) &=& \frac{1}{n}\sum_{i \leq n} |u_{i}(t) - y_{i}| \nonumber \\
  &\leq& \frac{\sqrt{n}}{n}\|\*u(t) - \*y\| \nonumber \\
  &\leq& O\left(\frac{1}{\sqrt{n}}\right) \label{eq:lossBound@k}
 \end{eqnarray}
 We get \eqref{eq:lossBound@k}, because $\|\*u(t) - \*y\| \leq (1-\frac{\eta\lambda_{0}}{2})^{t} \cdot O(n) \leq \frac{1}{2}$ for $k = \Omega(\frac{1}{\eta\lambda_{0}}\log(n))$. Next, we know that $\|\*w_{r}(t) - \*w_{r}(0)\| \leq R$, $\forall r \in [m]$ and $\|\*B(t) - \*B(0)\| \leq \tau$, where $R \leq \frac{n}{\sqrt{m}d\lambda_{0}\delta}$ and $\tau \leq O\left(\sqrt{\frac{n}{\lambda_{0}}}\right)$. For all $i$, $\tau_{i} = i$ such that,
 \begin{equation*}
     \@{R}_{S}(\@{F}_{R,\tau_{i}}^{\*B(0)}) \leq \frac{\tau_{i}}{\sqrt{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)}.
 \end{equation*}
 Let $i^{*}$ is such that, $\tau \leq \tau_{i^{*}}$, so $i^{*} = O\left(\sqrt{\frac{n}{\lambda_{0}}}\right)$. Now,
 \begin{eqnarray}
  \@{R}_{S}(\@{F}_{R,\tau_{i^{*}}}^{\*B(0)}) &\leq& \frac{\tau_{i^{*}}}{\sqrt{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)} \nonumber \\
  &\leq& \frac{\tau_{i}+1}{\sqrt{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)} \nonumber \\ 
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) \nonumber \\
  &+& \frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{\sqrt{nd}m^{1/4}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) + 2R^{2}\sqrt{\frac{m}{\pi}} \nonumber \\
  &+& R\sqrt{\log(2/\delta)} \nonumber \\ 
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}}\left(1 + \left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) \nonumber \\
  &+& \frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}} + 2R^{2}\sqrt{\frac{m}{\pi}} + R\sqrt{\log(2/\delta)} \nonumber  \\
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}}+\sqrt{\frac{n\lambda_{0}^{-1}}{nd}}\left(1\left(\frac{4\log(2/\delta)}{m}\right)^{1/4}\right) \nonumber \\
  &+& O\left(\frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}}\right) \nonumber  \\
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}} + O\left(\frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}}\right) \nonumber  
 \end{eqnarray}
 Now we use the following theorem to bound generalization error.
 \begin{theorem}
  Let $\mathcal{L}$ be a loss function bounded by $(0,c)$ and is $\rho$-Lipschitz in the first argument. Then with probability $1-\delta$ over a sample $S$ of size $n$ from $\mathcal{D}$,
  \begin{equation*}
    \sup_{f \in \@{F}}\{\@{L}_{\@{D}}(f) - \@{L}_{S}(f)\} \leq 2\rho\@{R}_{S}(\@{F}) + 3c\sqrt{\frac{\log(2/\delta)}{2n}} 
  \end{equation*}
 \end{theorem}
 Now from the theory of Rademacher complexity and taking a union bound over a finite set of $i$'s for any random initialization $\*B(0)$. for a sample $S$ we have the following with at least $1-\delta$ probability. 
 \begin{equation*}
   \sup_{f \in \@{F}_{R,\tau_{i^{*}}}^{\*B(0)}}\{\@{L}_{\@{D}}(f) - \@{L}_{S}(f)\} \leq 2\rho\@{R}_{S}(\@{F}_{R,\tau_{i^{*}}}^{\*B(0)}) + O\left(\sqrt{\frac{\log(\frac{n}{\lambda_{0}\delta})}{2n}}\right)
 \end{equation*}
 This implies that for all $f \in \@{F}_{R,\tau_{i^{*}}}^{\*B(0)}$,
 \begin{eqnarray}
  \@{L}_{\@{D}}(f) &\leq& \@{L}_{S}(f) + 2\rho\@{R}_{S}(\@{F}_{R,\tau_{i^{*}}}^{\*B(0)}) + O\left(\sqrt{\frac{\log(\frac{n}{\lambda_{0}\delta})}{2n}}\right) \nonumber \\
  &\leq& \frac{1}{\sqrt{n}} + 2\rho\@{R}_{S}(\@{F}_{R,\tau_{i^{*}}}^{\*B(0)}) + O\left(\sqrt{\frac{\log(\frac{n}{\lambda_{0}\delta})}{2n}}\right) \nonumber \\
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}} + O\left(\frac{\mbox{poly}(n,d^{-1},\lambda_{0}^{-1},\delta^{-1})}{m^{1/4}}\right) + O\left(\sqrt{\frac{\log(\frac{n}{\lambda_{0}\delta})}{2n}}\right) \nonumber \\
  &\leq& \sqrt{\frac{(\*y-\*u(0))^{T}(\*H^{\infty})^{-1}(\*y-\*u(0))}{nd}} + O\left(\sqrt{\frac{\log(\frac{n}{\lambda_{0}\delta})}{2n}}\right) \nonumber
 \end{eqnarray}
\end{proof}

==> sections/new-neurons.tex <==
\newcommand{\nir}[1]{{\color{red} #1}}
\section{Reducing The Number of Neurons}
The matrix $\*W$ is the first layer parameters. 
% It is important to note that the number of neurons in our architecture is $m$ and here we take advantage of dependencies between them. 
% \nir{How can it be important that the number of neurons is $m$?}
% {\color{red} Claiming that you the neurons have some kind of interdependence is very vague and not clear.  You are not really explaining what this interdependence is anywhere.  You are just replacing the input to the neurons from a low dimensional space.}
We represent this weight matrix $\*W$ as the product
%Hence, we can represent the weight matrix $\*W = 
$\*B\*C$. Here $\*B \in \~R^{k \times \ell}$ and same as before, $\*C \in \~R^{\ell \times d}$.
The final layer is represented as $\nu \in \~R^{k}$, where $\nu = \*v\*A$. Here $\*A \in \~R^{m \times k}$. In other words, we add a dimension reduction gadget as input to the final layer. We study the effect of this addition on the NTK bound.
%During the gradient descent process for every input, not all the neurons change its activation function value in each gradient descent update stage. As a result in the linear model, the change in the weight matrix $\*W$ has a low rank structure. In this section we show how can we take advantage of this fact and reduce the number of parameters that are required to be learnt.

%\subsection{Training}
Now we discuss how this affects the training phase. First we randomly and independently initialize $\*A \in \~R^{m \times k}$ such that all its entries are iid sampled from $\@{N}(0,1/\sqrt{k})$ for some $k < m$. We also initialize $\*C$ as mentioned in the previous section. Next, recall that $\*v$ is initialized as a random vector sampled from $\{-1,+1\}^{m}$. Now, we learn $\*B$ using gradient descent on the loss function $\Phi(\*B) = \frac{1}{2}\|\*y - \*u\|^{2}$ based on a small learning rate $\eta$ by keeping rest of the network parameters fixed. The matrix $\*B$ is updated as follows,
% Every entry of $\*C$ are sampled from $\@{N}(0,1/\sqrt{d\ell})$ where $\ell$ is $O(\log(n))$. Next we sample $\*v \sim \mbox{Unif}\{-1,1\}^{m}$. 
% These parameters are fixed during the entire GD process. For some learning rate $\eta > 0$ we update every row of $\*B$ as follows,

\begin{eqnarray*}
  \*B(t+1) &=& \*B(t) - \eta\frac{\partial \Phi(\*B(t))}{\partial \*B(t)} \\
  &=& \*B(t) - \frac{\eta}{\sqrt{m}}\sum_{j \leq n}(\*y_{j} - \*u_{j}(t))\*A^{T}\*Z_{j}(t)\*X_{j}\*C^{T}\ .
\end{eqnarray*}

Here $\*Z_{j}(t) \in \{-1,0,1\}^{m}$ is such that its $r^{th}$ index is $\*v_{r}\cdot\mathbbm{1}\{\*A_{r}\*B(t)\*C\*X_{j}^{T} > 0\}$ for all $r \in [m]$. Now given the input $\*X$, the gram matrix $\*H^{\infty} \in \~R^{n \times n}$ is defined with its $(i,j)^{th}$ term  as follows:
\begin{equation}
  \*H_{i,j}^{\infty} = \~E_{\*B}\left[\frac{1}{m}(\*X_{i}\*C^{T}\*C\*X_{j}^{T})(\*Z_{i}\*A\*A^{T}\*Z_{j}^{T})\right]\ .
\end{equation}

Note that $\*Z_{i}$ and $\*Z_{j}$ are random because they depend on $B$.
%Note that the randomness are in the $\*Z_{i}$ and $\*Z_{j}$ vectors due to $\*B$, whose entries are independent and identically distributed random samples from $\@{N}(0,1)$. 

Now for a random $\*B(0)$ upon initialization, we define $\*H(0) \in \~R^{n \times n}$  by $\forall i,j \in [n]$:

\begin{equation}{\label{eq:ker2}}
  \*H_{i,j}(0) = \frac{1}{m}(\*X_{i}\*C^{T}\*C\*X_{j}^{T}) (\*Z_{i}(0)\*A\*A^{T}\*Z_{j}^{T}(0))\ .
\end{equation}

% \begin{lemma}
%  With at least $1-\delta$ probability,
%  \begin{equation*}
%   \|\*H^{\infty} - \*H(0)\| \leq O\left(\frac{n^{2}\log(n/\delta)}{2md}\right)
%  \end{equation*}
% \end{lemma}
% We prove it using Hoeffding's inequality. The details are discussed in the appendix. 

\begin{lemma}{\label{lemma:ConditionalEvent}}
 If $\*B \in \~R^{k \times \ell}$ is a random matrix whose entries are iid sample from $\@{N}(0,1)$ then with probability $1-\delta$ the following holds.
 
 For any $\*B(0)$, if $\|\*A_{r}\*B\*C - \*A_{r}\*B(0)\*C\| \leq O\left(\frac{\delta^{2}\lambda_{0}}{n^{2}}\right) \stackrel{\Delta}{=} R$ then with $\*B$ the matrix $\*H \in \~R^{n \times n}$ whose $(i,j)^{th}$ entries are defined \eqref{eq:ker2},
 satisfies $\|\*H - \*H(0)\| \leq \frac{\lambda_{0}}{4}$ and $\lambda_{\min}(\*H) \geq \frac{\lambda_{0}}{4}$.
\end{lemma}
% \nir{This lemma is structured like " if....then...if....then...."  While it is logically possible to write such statements (this is often done, though discouraged in computer languages like Python), no reviewer is going to accept this, and I doubt that you meant to do this on purpose.  Also I don't understand what is the matrix $\*B$, I only understand what $\*B(0)$ is.}
\begin{proof}
 For a fixed $\*A, \*C$ and a random $\*B$ we get a random vector as $\*W_{r} = \*A_{r}\*B\*C$. Similarly we also define $\*W_{r}(0)$ corresponding to $\*B(0)$. Now consider the following event for every input $\*X_{i} \in \*X$ and neuron $r \in [m]$,
 \begin{equation*}
   \@{E}_{r,i} = \{\exists \*B : \|\*W_{r} - \*W_{r}(0)\| \leq R, \mathbbm{1}\{\*W_{r}(0)\*X_{i}^{T} \geq 0\} \neq \mathbbm{1}\{\*W_{r}\*X_{i}^{T} \geq 0\}\}.
 \end{equation*}
 The above event happens if and only if $|\*W_{r}(0)\*X_{i}^{T}| \leq R$. Now notice that for a fixed $\*A_{r},\*C$ and a randomly initialized $\*B(0)$ we have $h \sim \@{N}(0,1)$ where $h = \*A_{r}\*B(0)\*C\*X_{i}^{T}$. So $\~P(\@{E}_{r,i}) = \~P(|h| \leq R) \leq \int_{-R}^{R}\frac{1}{\sqrt{2\pi}}\exp(-x^{2})dx \leq R$. Now we bound deviation of every entry $(i,j) \in [n] \times [n]$ as follows,
 \begin{eqnarray*}
  \~E[|\*H_{i,j} - \*H_{i,j}(0)|] &=& \~E\left[\frac{1}{m}\left|(\*X_{i}\*C^{T}\*C\*X_{j}^{T})(\*Z_{i}\*A\*A^{T}\*Z_{j}^{T} - \*Z_{i}(0)\*A\*A^{T}\*Z_{j}^{T}(0))\right|\right] 
%   &=& \~E\left[\frac{1}{m}(\*X_{i}\*C^{T}\*C\*X_{j}^{T})((\*Z_{i} - \*Z_{i}(0))\*A\*A^{T}\*Z_{j}^{T} + \*Z_{i}(0)\*A\*A^{T}(\*Z_{j} - \*Z_{j}^{T}(0)))\right] \\
%   &\leq& \~E\left[\frac{2}{m}\|(\*Z_{i} - \*Z_{i}(0))\*A\*A^{T}\| \|\*Z_{j}\| + \|\*Z_{i}(0)\| \|\*A\*A^{T}(\*Z_{j} - \*Z_{j}^{T}(0))\|\right] \\
%   &\leq& \~E\left[\frac{2\sqrt{m}}{m}\|(\*Z_{i} - \*Z_{i}(0))\*A\*A^{T}\| + \|\*A\*A^{T}(\*Z_{j} - \*Z_{j}^{T}(0))\|\right]
 \end{eqnarray*}
%  \nir{The left hand side has absolute value, while the right hand side doesn't.  is this a mistake?}
 Now notice that,
 \begin{eqnarray*}
  (\*Z_{i}\*A\*A^{T}\*Z_{j}^{T} - \*Z_{i}(0)\*A\*A^{T}\*Z_{j}^{T}(0)) &=& \sum_{p,q}\*Z_{i,p}\*M_{p,q}\*Z_{j,q} - \*Z_{i,p}(0)\*M_{p,q}\*Z_{j,q}(0) \\
  &=&\sum_{p,q}\*M_{p,q}\*v_{p}\*v_{q}(\mathbbm{1}(\*A_{p}\*B\*C\*X_{i}^{T} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B\*C\*X_{j}^{T} \geq 0) \\
  &-& \mathbbm{1}(\*A_{p}\*B(0)\*C\*X_{i}^{T} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B(0)\*C\*X_{j}^{T} \geq 0)) 
 \end{eqnarray*}
 
 Here $\*M_{p,q}$ is the inner product between the $p^{th}$ and the $q^{th}$ row of $\*A$, i.e., $\*M_{p,q} = \*A_{p}\*A_{q}^{T}$. Next, since $\~E[|\mathbbm{1}(\*A_{p}\*B\*C\*X_{i} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B\*C\*X_{j} \geq 0) - \mathbbm{1}(\*A_{p}\*B(0)\*C\*X_{i} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B(0)\*C\*X_{j} \geq 0)|] \leq \~P(\@{E}_{p,i}) + \~P(\@{E}_{q,j})$, hence $\mathbbm{1}(\*A_{p}\*B\*C\*X_{i} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B\*C\*X_{j} \geq 0) - \mathbbm{1}(\*A_{p}\*B(0)\*C\*X_{i} \geq 0)\cdot \mathbbm{1}(\*A_{q}\*B(0)\*C\*X_{j} \geq 0)$ is either $-1$ or $1$ with probability at most $2R$. Here the randomness is due to the random matrix $\*B$. So we can rewrite, $(\*Z_{i}\*A\*A^{T}\*Z_{j}^{T} - \*Z_{i}(0)\*A\*A^{T}\*Z_{j}^{T}(0)) = \*x\*A\*A^{T}\*y$ where $\*x$ and $\*y$ are $m$ dimensional vectors such that with at least $1-\delta/2$ probability $\|\*x\|^{2} = \|\*y\|^{2} \leq 
 \frac{2mR}{\delta}$. 
    % \nir{In the above text, when you talk about probability, it is not clear which probability space you mean.  Are you holding A,C,v fixed and putting probabilities on B only?}
 We use the following claim, to discuss the desired property of $\*A$.
 \begin{claim}{\label{claim1}}
   Let $\@{S}$ be a set such that every element $\*s \in \@S$ is an $m$ dimensional vector in $\{-1,0,+1\}^{m}$ and $\|\*s\|_{1} \leq \frac{2mR}{\delta}$. The size of such set $|\@{S}| = O(\binom{m}{mR/\delta}\cdot 3^{mR/\delta})$. Let $k = O(\log(|\@{S}|)) = \tilde{O}\left(\frac{mR}{\delta}\right)$ and recall matrix $\*A$ has random i.i.d. samples from $\@N(0,1/\sqrt{k})$. Now for all $\*s \in \@S$ we get, $\|\*s\*A\| = O(\|\*s\|) = O(\sqrt{mR/\delta})$ with high probability.

 \end{claim}
 
  Now the above claim yields, $\~E[|\*H_{i,j} - \*H_{i,j}(0)|] \leq \frac{1}{m}(O(1)\sqrt{mR/\delta}\sqrt{mR/\delta}) = O(R/\delta)$. So, $\~E[\sum_{i,j}|\*H_{i,j} - \*H_{i,j}(0)|] \leq O\left(\frac{n^{2}R}{\delta}\right)$ and by Markov inequality we have $\sum_{i,j}|\*H_{i,j} - \*H_{i,j}(0)| \leq O\left(\frac{n^{2}R}{\delta^{2}}\right)$ with at least $1-\delta$ probability. Therefore with at least $1-\delta$ probability $\|\*H - \*H(0)\| \leq O\left(\frac{n^{2}R}{\delta^{2}}\right)$. Finally,
 \begin{equation*}
   \lambda_{\min}(\*H) \geq \lambda_{\min}(\*H(0)) - O\left(\frac{n^{2}R}{\delta^{2}}\right) \geq \frac{\lambda_{0}}{2}
 \end{equation*}
\end{proof}

Note that the above lemma ensures that $R = O\left(\frac{\lambda_{0}\delta^{2}}{n^{2}}\right)$. Further, it implies that from the point of initialization of $\*B(0)$, out of $m$ neurons only $O\left(\frac{mR}{\delta}\right)$ of them change their activation function value from their initial function value. The next lemma states the required learning rate $\eta$ and the number of neurons $m$ to get a desired training error after certain iterations. 

\begin{theorem}{\label{thm:train}}
 Assume $\lambda_0 = \lambda_{\min}(\*H^{\infty}) > 0$. For $\delta \in (0,1)$, number of neurons $m = \Omega\left(\frac{n^{6}}{\lambda_{0}^{4}\delta^{7}}\right)$, $\*B(0)$ is randomly initialized and we set $\eta = O\left(\frac{\lambda_{0}\delta^{4}}{n^{2}}\right)$. Then during  gradient descent we have the following with probability at least $1-\delta$ for $t = 0, 1, \ldots$,
 \begin{equation}
   \|\*u(t) - \*y\|^{2} \leq \left(1-\frac{\eta\lambda_{0}}{2}\right)^{t}\|\*u(0) - \*y\|^{2}
 \end{equation} 
\end{theorem}

\begin{proof}
 We prove this by induction. The induction hypothesis is the following,
 \begin{equation}
   \|\*u(t) - \*y\|^{2} \leq \left(1-\frac{\eta\lambda_{0}}{2}\right)^{t}\|\*u(0) - \*y\|^{2}
 \end{equation}

% The following corollary follows from the hypothesis.
% \begin{corollary}{\label{cor:neronSimple}}
%  If the above hypothesis is true then we have the following for all $r \in [m]$.
%   \begin{equation}
%   \|\*w_{r}(t+1) - \*w_{r}(0)\| \leq \frac{4\sqrt{n}\|\*u(0) - \*y\|}{\sqrt{m}d\lambda_{0}} \stackrel{\Delta}{=} R'
%  \end{equation}
% \end{corollary}

% \begin{proof}

%  \begin{eqnarray}
%   \|\*w_{r}(t+1) - \*w_{r}(0)\| &\leq& \sum_{t' \leq t}\left\|-\eta\frac{\partial \Phi(\*B(t'))}{\partial \*b_{r}(t')}\*C\right\| \nonumber \\
%   &=& \eta\sum_{t' \leq t}\left\|\sum_{j \leq n}\frac{(y_{j} - u_{j}(t'))v_{r}\*x_{j}\*C^{T}\*C(\mathbbm{1}\{\*b_{r}(t')\*C\*x_{j}^{T} \geq 0\})}{\sqrt{m}} \right\| \nonumber \\
%   &\leq& \eta\sum_{t' \leq t}\left\|\sum_{j \leq n}\frac{(y_{j} - u_{j}(t'))\*x_{j}\*C^{T}\*C}{\sqrt{m}} \right\| \label{eq:cor4eq1} \\
%   &\leq& \frac{\eta}{\sqrt{m}}\sum_{t' \leq t}\left(\sum_{j \leq n}|y_{j} - u_{j}(t')|\right)\max_{j}\|\*x_{j}\*C^{T}\*C\| \label{eq:cor4eq2} \\
%   &\leq& \frac{\eta}{\sqrt{m}d}\sum_{t' \leq t}\left(\sum_{j \leq n}|y_{j} - u_{j}(t')|\right) \label{eq:cor4eq3} \\
%   &\leq& \frac{\eta}{\sqrt{m}d}\sum_{t' \leq t}\sqrt{n}\|\*y - \*u(t')\| \label{eq:cor4eq4} \\
%   &\leq& \frac{\eta\sqrt{n}}{\sqrt{m}d}\sum_{t' \leq t}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \label{eq:cor4eq5} \\
%   &\leq& \frac{\eta\sqrt{n}}{\sqrt{m}d}\sum_{t'=0}^{\infty}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \nonumber \\
%   &=& \frac{4\sqrt{n}\|\*u(0) - \*y\|}{\sqrt{m}d\lambda_{0}} \nonumber
%  \end{eqnarray}

% In \eqref{eq:cor4eq1} we upper bound $\mathbbm{1}\{\*b_{r}(t')\*C\*x_{j}^{T} \geq 0\}$ by $1$. In \eqref{eq:cor4eq2} we used holder's inequality. In \eqref{eq:cor4eq3} we use the upper bound $|\*x_{i}\*C^{T}\*C| \leq 1/d$. Using Cauchy–Schwartz we get \eqref{eq:cor4eq4}. In \eqref{eq:cor4eq5} we used our hypothesis. 
% \end{proof}

Notice that the hypothesis is trivially true for the base case $t = 0$. Suppose it holds true for $t' = 0, 1, \ldots, t$ and now we show that it also holds for $t' = t+1$. We have,
\begin{eqnarray*}
  \|\*u(t+1) - \*u(t)\|^{2} &\leq& \eta^{2}\sum_{i \leq n} \left(\frac{\partial \*u_{i}(t)}{dt} \right)^{2} \nonumber \\
  &\leq& \eta^{2}\sum_{i \leq n} \left(\sum_{j \leq n}\frac{1}{m}(\*y_{j} - \*u_{j}(t))(\*X_{i}\*C^{T}\*C\*X_{j}^{T})(\*Z_{i}(t)\*A\*A^{T}\*Z_{j}^{T}(t))\right)^{2} \nonumber \\
  &\leq& \eta^{2}n \left(\frac{1}{m}\max_{j} |\*X_{i}\*C^{T}\*C\*X_{j}^{T}|\sum_{j \leq n}\left|(\*Z_{i}(t)\*A^{T}\*A\*Z_{j}^{T}(t)) \left(\*y_{j} - \*u_{j}(t)\right)\right| \right)^{2} \nonumber \\
  &\leq& \eta^{2}n \left(\frac{O(1)}{m}\left(\sum_{j \leq n}(\*Z_{i}(t)\*A\*A^{T}\*Z_{j}^{T}(t))^{2}\right)^{1/2} \|\*y - \*u(t)\| \right)^{2} \nonumber \\
  &\leq& \eta^{2}n \left(\frac{O(1)}{m}\left(\sum_{j \leq n}(\|\*Z_{i}(t)\*A\|\|\*A^{T}\*Z_{j}^{T}(t)\|)^{2}\right)^{1/2} \|\*y - \*u(t)\| \right)^{2} \nonumber
\end{eqnarray*}

Notice that,
\begin{eqnarray*}
 \|\*Z_{i}(t)\*A\|^{2} = \sum_{r_{1} \leq k} (\*Z_{i}(t)\*A_{r_{1}}^{T})^{2} = \sum_{r_{1} \leq k}\left(\sum_{r_{2} \leq m}\*v_{r_{2}}\mathbbm{1}(\*A_{r_{2}}\*B(t)\*C\*X_{i}^{T} \geq 0)\*A_{r_{2},r_{1}}\right)^{2} 
 = \sum_{r_{1} \leq k}(\*v\tilde{\*A}_{r_{1}}^{T})^{2} = \|\*v\tilde{\*A}\|^{2}
\end{eqnarray*}

Here $\tilde{\*A}_{r_{1}}$ represents the entrywise vector product between $\*A_{r_1}$ and corresponding indicator variable. Notice that $\|\tilde{\*A}\|_{F}^{2} \leq \|\*A\|_{F}^{2}$ and with at least $1-\delta/2$ probability $\|\*A\|_{F}^{2} \leq 2m/\delta$. So, for all $i \in [n]$, $\~E_{\*v}[\|\*Z_{i}(t)\*A\|^{2}] = \sum_{r_{1}}\|\tilde{\*A}_{r_{1}}\|^{2} \leq \|\*A\|_{F}^{2} \leq 2m/\delta$. Now by Markov we get, $\sum_{i}\|\*Z_{i}(t)\*A\|^{2} \leq O(nm/\delta^{2})$ with at least $1-\delta$ probability. Now,

\begin{eqnarray*}
  \|\*u(t+1) - \*u(t)\|^{2} &\leq& \eta^{2}n \left(\frac{O(1)}{m}\left(\sum_{j \leq n}(\|\*Z_{i}(t)\*A^{T}\|\|\*A\*Z_{j}^{T}(t)\|)^{2}\right)^{1/2} \|\*y - \*u(t)\| \right)^{2} \nonumber \\
  &\leq& \eta^{2}n \left(\frac{O(1)}{m}\left(\frac{nm^{2}}{\delta^{4}}\right)^{1/2} \|\*y - \*u(t)\| \right)^{2} 
  \leq O\left(\frac{\eta^{2}n^{2}}{\delta^{4}}\right) \|\*y - \*u(t)\|^{2} \nonumber
\end{eqnarray*}

From the above analysis notice that,
\begin{eqnarray}
 |\*u_{i}(t+1) - \*u_{i}(0)| &\leq& \sum_{t' < t}\left|\frac{\partial \*u_{i}(t')}{dt'} \right| \nonumber \\
  &\leq& O\left(\frac{\eta}{\delta^{2}}\right) \sum_{t' < t}\sqrt{n}\|\*y - \*u(t)\| \label{eq} \\
  &\leq& O\left(\frac{\eta\sqrt{n}}{\delta^{2}}\right) \sum_{t' < t}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \nonumber \\
  &\leq& O\left(\frac{\eta\sqrt{n}}{\delta^{2}}\right) \sum_{t' = 1}^{\infty}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \nonumber \\
  &\leq& \frac{\sqrt{n}}{\delta^{2}\lambda_{0}}\|\*u(0) - \*y\| \leq \frac{n}{\delta^{5/2}\lambda_{0}} \nonumber
\end{eqnarray}

Our network parameters at time $t = 0$, ensures that the output $\*u_{i}(0)$ is $O(1)$, for all $i \in [n]$. Further we know that $\*y_{i} = O(1)$. Hence by Markov's inequality we have $\|\*u(0) - \*y\|^{2} \leq n/\delta$ with at least probability $1-\delta$.

Now, based on the events $\@{E}_{r,i}$ for all input $\*X_{i}$ and neuron $r$, let $\*u_{i}$ be the network output for $\*X_{i}$. Then $|\*u_{i} - \*u_{i}(0)| = \frac{1}{\sqrt{m}}\*v(\sigma(\*W\*X_{i}^{T}) - \sigma(\*W(0)\*X_{i}^{T})) \leq \frac{1}{\sqrt{m}}\|\*v\|\|\*W - \*W(0)\|\|\*X_{i}\| \leq \frac{1}{\sqrt{m}} \sqrt{m} \sqrt{m}R = \sqrt{m}R$. Now in order to insure that the condition in lemma \ref{lemma:ConditionalEvent} holds, we need ensure $|\*u_{i}(t+1) - \*u_{i}(0)| \leq |\*u_{i} - \*u_{i}(0)|$. So we get, $m = \Omega\left(\frac{n^{6}}{\lambda_{0}^{4}\delta^{7}}\right)$. Further, we know that, $R = O\left(\frac{\delta^{2}\lambda_{0}}{n^{2}}\right)$ and $\~P(\@{E}_{r,i}) \leq R$. Let $\*S_{i} = \{r \in [m]: \mathbbm{1}\{\@{E}_{r,i}\} = 0\}$ and $\*S_{i}^{\perp} = [m] \backslash \*S_{i}$. Let $\*s_{i} \in \~R^{m}$ be such that $\*s_{i,r} = 1, \forall r \in [\*S_{i}^{\perp}]$. So, $\~E[\|\*s_{i}\|^{2}] \leq mR$. Further, $\~E[\sum_{i \leq n}|\*S_{i}^{\perp}|] \leq mnR$. So by using Markov inequality we have $\sum_{i \leq n}|\*S_{i}^{\perp}| \leq \frac{mnR}{\delta}$ with at least $1-\delta$ probability. Now consider the following term,
\begin{eqnarray}
 \*u_{i}(t+1) - \*u_{i}(t) &=& \frac{1}{\sqrt{m}}\sum_{r \leq m}\*v_{r}\left[\sigma(\*A_{r}\*B(t+1)\*C\*X_{i}^{T}) - \sigma(\*A_{r}\*B(t)\*C\*X_{i}^{T})\right] \nonumber \\
 &=& \frac{1}{\sqrt{m}}\sum_{r \leq m}\*v_{r}\left[\sigma\left(\*A_{r}\left(\*B(t) - \eta\frac{\partial \Phi(\*B(t))}{\partial \*B(t)}\right)\*C\*X_{i}^{T}\right) - \sigma(\*A_{r}\*B(t)\*C\*X_{i}^{T})\right] \nonumber \\
 &=& I^{i}_{1} + I^{i}_{2} \nonumber
\end{eqnarray}

We analyze the term based on two sets of neurons. We have $I^{i}_{1}$ corresponding to the neurons which do not change their activation function value based for the network parameter $\*B(t)$ and $\*B(t+1)$. The term $I^{i}_{2}$ corresponds to rest of the neurons (that changes).
\begin{eqnarray}
 I^{i}_{1} &=& \frac{1}{\sqrt{m}}\sum_{r \in \*S_{i}}\*v_{r}\left[\sigma\left(\*A_{r}\left(\*B(t) - \eta\frac{\partial \Phi(\*B(t))}{\partial \*B(t)}\right)\*C\*X_{i}^{T}\right) - \sigma(\*A_{r}\*B(t)\*C\*X_{i}^{T})\right] \nonumber \\
 I^{i}_{2} &=& \frac{1}{\sqrt{m}}\sum_{r \in \*S_{i}^{\perp}}\*v_{r}\left[\sigma\left(\*A_{r}\left(\*B(t) - \eta\frac{\partial \Phi(\*B(t))}{\partial \*B(t)}\right)\*C\*X_{i}^{T}\right) - \sigma(\*A_{r}\*B(t)\*C\*X_{i}^{T})\right] \nonumber
\end{eqnarray}

First we upper bound $I^{i}_{2}$.
\begin{eqnarray}
 |I^{i}_{2}| &=& \left|\frac{1}{\sqrt{m}}\sum_{r \in \*S_{i}^{\perp}}\*v_{r}\left[\sigma\left(\*A_{r}\left(\*B(t) - \eta\frac{\partial \Phi(\*B(t))}{\partial \*B(t)}\right)\*C\*X_{i}^{T}\right) - \sigma(\*A_{r}\*B(t)\*C\*X_{i}^{T})\right]\right| \nonumber \\
 &\leq& \left|\frac{1}{\sqrt{m}}\sum_{r \in \*S_{i}^{\perp}}\left[ - \eta\*A_{r}\left(\frac{\partial \Phi(\*B(t))}{\partial \*B(t)}\right)\*C\*X_{i}^{T} \right]\right| \label{eq:thm1eq1} \\
%  &\leq& \frac{\eta}{\sqrt{m}}\left\|\sum_{r \in \*S_{i}^{\perp}}\frac{\partial \Phi(\*B(t))}{\partial \*b_{r}(t)}\right\|\|\*C\*x_{i}^{T}\| \nonumber \\
%  &\leq& \frac{\eta}{\sqrt{m}d}|\*S_{i}^{\perp}|\max_{r \in \*S_{i}^{\perp}}\left\|\frac{\partial \Phi(\*B(t))}{\partial \*b_{r}(t)}\right\| \nonumber \\
 &\leq& \frac{\eta}{\sqrt{m}}\|\*s_{i}\|\cdot\left\|\sum_{j \leq n}\frac{(\*y_{j}-\*u_{j}(t))(\*X_{j}\*C^{T}\*C\*X_{i}^{T})(\*A_{\*S_{i}^{\perp}}\*A^{T}\*Z_{j}^{T}(t))}{\sqrt{m}}\right\| \label{eq:thm1eq2} \\
 &\leq& \eta \sqrt{\frac{mR}{m\delta}}\left\|\sum_{j \leq n}\frac{(\*y_{j}-\*u_{j}(t))(\*X_{j}\*C^{T}\*C\*X_{i}^{T})(\*A_{\*S_{i}^{\perp}}\*A^{T}\*Z_{j}^{T}(t))}{\sqrt{m}}\right\| \nonumber \\
 &\leq& \eta\sqrt{\frac{R}{m\delta}}\left\|\max_{j}(\*X_{j}\*C^{T}\*C\*X_{i}^{T})(\*A_{\*S_{i}^{\perp}}\*A^{T}\*Z_{j}^{T}(t))\right\|\sum_{j \leq n}|\*y_{j}-\*u_{j}(t)| \label{eq:thm1eq3} \\
 &\leq& \eta\sqrt{\frac{R}{m\delta}}\left\|\max_{j}\*A_{\*S_{i}^{\perp}}\*A^{T}\*Z_{j}^{T}(t)\right\|\sqrt{n}\|\*y-\*u(t)\| \nonumber \\
 &\leq& \eta\sqrt{\frac{nR}{m\delta}}\|\*A_{\*S_{i}^{\perp}}\|\|\*A\|\max_{j}\|\*Z_{j}(t)\|\|\*y-\*u(t)\| \nonumber \\
 &\leq& \eta\sqrt{\frac{nR}{m\delta}}\sqrt{\frac{m}{k}}\sqrt{m}\|\*y-\*u(t)\| \label{eq:thm1eq4} \\
 &\leq& \eta\sqrt{\frac{n}{\delta}}\|\*y-\*u(t)\| \nonumber
\end{eqnarray}
Since ReLU is a $1$-Lipschitz function and $|\*v_r| = 1$,  we get \eqref{eq:thm1eq1}. We have \eqref{eq:thm1eq2} by applying Cauchy-Schwartz on the sum over $|\*S_{i}^{\perp}|$ terms. We get \eqref{eq:thm1eq3} due to Holder inequality. The $\*A_{\*S_{i}^{\perp}}$ is a $m \times d$ dimensional matrix. Here every row of this matrix is either all zero vector or a row from $\*A$. For all $j \in [m]$, if $j \in \*S_{i}^{\perp}$, then the $j^{th}$ row of $\*A_{\*S_{i}^{\perp}}$ is equal to $\*A_{j}$, else it is $\{0\}^{k}$. So in \eqref{eq:thm1eq4} we upper bound $\|\*A_{\*S_{i}^{\perp}}\| \leq 1$. Further, $\|\*A\|^{2} \leq \frac{m}{k}$ and $\forall j \in [n], \|\*Z_{j}(t)\| \leq \sqrt{m}$. 

% Further, notice that,
% \begin{eqnarray*}
%  |\*u_{i}(t+1) - \*u_{i}(0)| &\leq& \sum_{t' < t} |\*u_{i}(t'+1) - \*u_{i}(t')| \\
%  &\leq& \frac{\eta \sqrt{nR}}{\delta}\sum_{t' < t}\|\*y-\*u(t')\| \nonumber \\
%  &\leq& \frac{\eta \sqrt{nR}}{\delta}\sum_{t' \leq t}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \label{eq:cor4eq5} \\
%  &\leq& \frac{\eta \sqrt{nR}}{\delta}\sum_{t'=0}^{\infty}\left(1-\frac{\eta\lambda_{0}}{2}\right)^{t'/2}\|\*u(0) - \*y\| \nonumber \\
%  &=& \frac{\sqrt{nR}\|\*u(0) - \*y\|}{\delta\lambda_{0}} \nonumber
% \end{eqnarray*}

% Now notice that the change in $\*u_{i}(t)$ is only due to $mR$ neurons. So the change with respect to one such neuron is $O\left(\frac{n^{3/2}\|\*u(0) - \*y\|}{m\delta\lambda_{0}}\right)$.

% At every step $t+1$, let 

% \begin{eqnarray}
%  \frac{4\sqrt{n}}{\sqrt{m}d\lambda_{0}}\|\*y - \*u(0)\| &\leq& =\frac{C\sqrt{d}\delta\lambda_{0}}{n^{2}} \\
%  \frac{4\sqrt{n}}{\sqrt{m}}O(\sqrt{\frac{n}{d}}) &\leq& \frac{Cd\sqrt{d}\delta\lambda_{0}^{2}}{n^{2}} \\
%  \frac{O(n)}{\sqrt{m}} &\leq& \frac{Cd^{2}\delta\lambda_{0}^{2}}{n^{2}} \\
%  \frac{O(n^{3})}{\sqrt{m}} &\leq& Cd^{2}\delta\lambda_{0}^{2} \\
%  m &\geq& O\left(\frac{n^{6}}{d^{4}\lambda_{0}^{4}\delta^{2}}\right)
% \end{eqnarray}

Now we express  $I^{i}_{1}$ as follows,
\begin{eqnarray}
 I^{i}_{1} &=& -\frac{\eta}{m}\sum_{j \leq n}(\*y_{j} - \*u_{j}(t))(\*X_{i}\*C^{T}\*C\*X_{j}^{T})\left(\sum_{r \in \*S_{i}}(\*Z_{i}(t)\*A_{r}^{T}\*A_{r}\*Z_{j}^{T}(t))\right) \nonumber \\
%  &=& -\frac{\eta}{m}\sum_{j \leq n}(\*y_{j} - \*u_{j}(t))(\*X_{i}\*C^{T}\*C\*X_{j}^{T})\left(\sum_{r \in \*S_{i}}(\*Z_{i}\*A_{r}^{T}(t)\*A_{r}(t)\*Z_{j}^{T}\right) \nonumber \\
 &=& -\eta\sum_{j \leq n}(\*y_{j} - \*u_{j}(t))(\*H_{i,j}(t) - \*H_{i,j}^{\perp}(t)) \nonumber
\end{eqnarray}

Here $\*H_{i,j}(t) = \*X_{i}\*C^{T}\*C\*X_{j}^{T}(\*Z_{i}(t)\*A\*A^{T}\*Z_{j}^{T}(t))$ and the term $\*H_{i,j}^{\perp}(t) = \*X_{i}\*C^{T}\*C\*X_{j}^{T}(\*Z_{i}(t)\*A_{\*S_{i}^{\perp}}\*A_{\*S_{i}^{\perp}}^{T}\*Z_{j}^{T}(t))$. $\*H^{\perp}$ is an $n \times n$ PSD matrix whose spectral norm can be bounded as follows,
\begin{eqnarray}
  \|\*H^{\perp}\| &\leq& \sum_{i,j}|\*H_{i,j}^{\perp}| = \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} \left|\*X_{i}\*C^{T}\*C\*X_{j}^{T}(\*Z_{i}(t)\*A_{\*S_{i}^{\perp}}\*A_{\*S_{i}^{\perp}}^{T}\*Z_{j}^{T}(t))\right|\right) \nonumber \\
  &\leq& \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} \left|O(1) \cdot (\*Z_{i}(t)\*A_{\*S_{i}^{\perp}}\*A_{\*S_{i}^{\perp}}^{T}\*Z_{j}^{T}(t))\right|\right) \nonumber \\
  &=& \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} \left|O(1) \cdot (\tilde{\*Z}_{i}(t)\*A_{\*S_{i}^{\perp}}\*A_{\*S_{i}^{\perp}}^{T}\tilde{\*Z}_{j}^{T}(t))\right|\right) \label{eq1} \\
  &\leq& \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} \left|O(1) \cdot \|\*A_{\*S_{i}^{\perp}}\tilde{\*Z}_{i}^{T}(t)\|\|\*A_{\*S_{i}^{\perp}}\tilde{\*Z}_{j}^{T}(t)\|\right|\right) \nonumber \\
  &\leq& \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} \left|O(1) \cdot \|\*A\tilde{\*Z}_{i}^{T}(t)\|\|\*A\tilde{\*Z}_{j}^{T}(t)\|\right|\right) \label{eq2} \\
  &\leq& \frac{1}{m}\sum_{i \leq n} \left(\sum_{j \leq n} O(1) \frac{mR}{\delta}\right) \nonumber \leq O\left(\frac{n^{2}R}{\delta}\right) \nonumber
\end{eqnarray}

In \eqref{eq1} the vectors $\tilde{\*Z}_{i}(t)$ and $\tilde{\*Z}_{j}(t)$ are $m$ dimensional sparse vectors. For every index of $r \in \*S_{i}^{\perp}$, $\tilde{\*Z}_{i,r}(t) = \*Z_{i,r}(t)$. Similarly the vector $\tilde{\*Z}_{j}(t)$ is also defined. So their sparsity is bounded by $|\*S_{i}^{\perp}|$. 

 $\tilde{\*Z}_{i}(t)$ and $\tilde{\*Z}_{j}(t)$. In \eqref{eq2} we use the upper bound $\|\*A_{\*S_{i}^{\perp}}\*Y^{T}\| \leq \|\*A\*Y^{T}\|$, where $\*Y \in \~R^{m}$.

Finally we bound our desired term,
\begin{eqnarray}
 \|\*y - \*u(t+1)\|^{2} &=& \|\*y - \*u(t) - (\*u(t+1) - \*u(t))\|^{2} \nonumber \\
 &=& \|\*y-\*u(t)\|^{2} + \|\*u(t+1) - \*u(t)\|^{2} - 2(\*y-\*u(t))^{T}(\*u(t+1) - \*u(t))\nonumber \\
 &=& \|\*y-\*u(t)\|^{2} + \|\*u(t+1) - \*u(t)\|^{2} - 2(\*y-\*u(t))^{T}\*I_{2}\nonumber \\
 &-& 2\eta(\*y-\*u(t))^{T}\*H(t)(\*y-\*u(t)) + 2\eta(\*y-\*u(t))^{T}\*H(t)^{\perp}(\*y-\*u(t)) \nonumber \\
 &\leq& \left(1 + \frac{\eta^{2}n^{2}}{\delta^{4}} - \sum_{i \leq n}2\eta\sqrt{\frac{n}{\delta}} - \eta\lambda_{0} + \frac{2\eta n^{2}R}{\delta}\right)\|\*y - \*u(t)\|^{2} \nonumber \\
 &\leq& \left(1 - \frac{\eta\lambda_{0}}{2}\right)\|\*y - \*u(t)\|^{2} \label{eq3} \\
 &\leq& \left(1 - \frac{\eta\lambda_{0}}{2}\right)^{t}\|\*y - \*u(0)\|^{2} \nonumber 
\end{eqnarray}

By setting $\eta = \frac{\lambda_{0}\delta^{4}}{2n^{2}}$ we get \eqref{eq3}.
\end{proof}

\paragraph{Running Time:} The previous theorem essentially implies that in an overparameterized network with network width of $O\left(\frac{n^6}{\lambda_{0}^4\delta^7}\right)$ one can find global minimum by gradient descent with a learning rate $\eta = O\left(\frac{\lambda_{0}\delta^{4}}{n^{2}}\right)$. However, notice that due to our dimensionality reduction, it can be achieved much faster even for network width of $O(n^{6})$. In each iteration we update a $k \times \ell$ dimensional matrix matrix $\*B$. For all $i \in [n]$ we do a matrix vector product, $\*Z_{i}(t)\*A$ and $\*X_{i}\*C^{T}$ which takes $O(mk + \ell d) = O\left(\frac{n^{10}}{\lambda_{0}^{7}\delta^{12}}\right)$. So each iteration of the gradient descent process takes $O\left(\frac{n^{10}}{\lambda_{0}^{7}\delta^{12}}\right)$. Now for $t \geq \frac{\log(\varepsilon)}{\log(1-\eta\lambda_{0})}$ our learnt parameter ensures,
\begin{equation*}
  \|\*y - \*u(t+1)\|^{2} \leq \varepsilon\cdot\|\*y - \*u(0)\|^{2}.
\end{equation*}

So the total running time to achieve this is $O\left(\frac{n^{11}\log(\varepsilon)}{\lambda_{0}^{7}\delta^{12}\log(1-\eta\lambda_{0})}\right)$. Notice that with existing technique the running time would be $O(nmdt)$ which is $O\left(\frac{n^{7}d\log(\varepsilon)}{\lambda_{0}^{4}\delta^{2}\log(1-(\lambda_{0}/n)^{2})}\right)$.

% In case of a full rank weigh matrix $\*W$,  the time taken to update $\*W(t+1)$ from $\*W(t)$ is $O(nmd)$, i.e., $O\left(\frac{n^{7}d}{\lambda_{0}^{4}\delta^{2}}\right)$. From $t \geq \frac{\log(\varepsilon)}{\log(1-c/n^{2})}$ our learnt parameter will ensure,
% \begin{equation*}
%   \|\*y - \*u(t+1)\|^{2} \leq \varepsilon\cdot\|\*y - \*u(0)\|^{2}
% \end{equation*}

% If $\*C$ is FJLT matrix then $\*C\*x_{i}^{T}$ takes $O(d\log(\ell))$ and $\*b_{r}\*C$ takes $O(d\ell\log(\ell))$. So the time taken to update $\*b_{r}(t+1)$ from $\*b_{r}(t)$ is $O(nd\ell\log(\ell))$. Finally, to update all $m$ rows of $\*B$ takes $O(mnd\ell\log(\ell))$, i.e., $O\left(\frac{n^{7}\log(n)^3}{d^{3}\lambda_{0}^{4}\delta^{2}}\right)$. From $t \geq \frac{\log(\veps)}{\log(1-cd/n^{2})}$ for some constant $c$ our learnt parameter will ensure,
% \begin{equation*}
%   \|\*y - \*u(t+1)\|^{2} \leq \veps\cdot\|\*y - \*u(0)\|^{2}
% \end{equation*}
